Synthetic Combinations: A Causal Inference Framework for Combinatorial Interventions

Consider a setting where there are $N$ heterogeneous units and $p$ interventions. Our goal is to learn unit-specific potential outcomes for any combination of these $p$ interventions, i.e., $N \times 2^p$ causal parameters. Choosing a combination of interventions is a problem that naturally arises in a variety of applications such as factorial design experiments, recommendation engines, combination therapies in medicine, conjoint analysis, etc. Running $N \times 2^p$ experiments to estimate the various parameters is likely expensive and/or infeasible as $N$ and $p$ grow. Further, with observational data there is likely confounding, i.e., whether or not a unit is seen under a combination is correlated with its potential outcome under that combination. To address these challenges, we propose a novel latent factor model that imposes structure across units (i.e., the matrix of potential outcomes is approximately rank $r$), and combinations of interventions (i.e., the coefficients in the Fourier expansion of the potential outcomes is approximately $s$ sparse). We establish identification for all $N \times 2^p$ parameters despite unobserved confounding. We propose an estimation procedure, Synthetic Combinations, and establish it is finite-sample consistent and asymptotically normal under precise conditions on the observation pattern. Our results imply consistent estimation given $\text{poly}(r) \times \left( N + s^2p\right)$ observations, while previous methods have sample complexity scaling as $\min(N \times s^2p, \ \ \text{poly(r)} \times (N + 2^p))$. We use Synthetic Combinations to propose a data-efficient experimental design. Empirically, Synthetic Combinations outperforms competing approaches on a real-world dataset on movie recommendations. Lastly, we extend our analysis to do causal inference where the intervention is a permutation over $p$ items (e.g., rankings).

==> archive/finite_sample_analysis_tightened_2.tex <==
\section{Theoretical Analysis}\label{sec:theoretical_analysis}
%
In this section, we establish finite-sample consistency of \method, starting with a discussion of the additional assumptions required for our results. 

\subsection{Additional Assumptions}\label{subsec:finite_sample_analysis_assumptions}
%
\begin{assumption}[Bounded Potential Outcomes]\label{ass:boundedness_potential_outcome}
We assume that $\E[Y_{n}^{(\pi)}] \in [-1,1]$ for any unit-combination pair $(n,\pi)$.
\end{assumption}
%
\begin{assumption}[Sub-Gaussian Noise]\label{ass:subgaussian_noise}
Conditioned on $\mathcal{A}$, for any unit-combination pair $(n,\pi)$, $\epsilon_n^{\pi}$ are independent zero-mean sub-Gaussian random variables with $\text{Var}[\epsilon_n^{\pi} ~ | ~  \mathcal{A}] \le \sigma^2$ and $\lVert \epsilon_n^{\pi} ~ | ~ \mathcal{A} \rVert_{\psi_2} \leq C\sigma$ for some constant $C > 0$. 
\end{assumption}
%
\begin{assumption} [Incoherence of Donor Fourier characteristics]
\label{ass:incoherence}
For every unit $u \in \mathcal{I}$, assume $\bchi(\Pi_u)$ satisfies incoherence:
$
\left\lVert \frac{\bchi(\Pi_u)^T\bchi(\Pi_u)}{|\Pi_u|} - \mathbf{I}_{2^p}\right\rVert_{\infty} \leq \frac{C'}{s}, 
$ for a universal constant $C' >0$. 
\end{assumption}
%
To define our next set of assumptions, we introduce necessary notation. For any subset of combinations $\Pi_S \subset \Pi$, let $\E[\bY_{\mathcal{I}}^{(\Pi_S)}] = [\E[\bY_u^{(\Pi_S)}]: u \in \mathcal{I}] \in \mathbb{R}^{|\Pi_S| \times |\mathcal{I}|}$.
%
\begin{assumption} [Donor Unit Balanced Spectrum]\label{ass:balanced_spectrum} For a given unit $n \in [N] \setminus \mathcal{I}$, let $r_n$ and $s_{1} \ldots s_{r_n}$ denote the rank and non-zero singular values of $ \E[\bY_{\mathcal{I}}^{(\Pi_n)} \ | \ \mathcal{A}]$, respectively. 
%
We assume that the singular values are well-balanced, i.e., for universal constants $c,c' > 0$, we have that $s_{r_n}/s_{1} \geq c$, and $\lVert \E[\bY^{(\Pi_n)}_{\mathcal{I}} ~ | ~ \mathcal{A} ]\rVert^2_F \geq c'|\Pi_n||\mathcal{I}|$.
\end{assumption}

\begin{assumption} [Subspace Inclusion]\label{ass:rowspace_inclusion} 
For a given unit $n \in [N] \setminus \mathcal{I}$ and intervention $\pi \in \Pi \setminus \Pi_n$,
assume that $\E[\bY^{(\pi)}_{\mathcal{I}}]$ lies within the row-span of $\E[\bY_{\mathcal{I}}^{(\Pi_n)}]$
\end{assumption}
%
\vspace{-2mm}
Assumption \ref{ass:incoherence} is necessary for finite-sample consistency when estimating $\balpha_n$ via the Lasso estimator \eqref{eq:Lasso_estimator}, and is commonly made when studying the Lasso \citep{rigollet2015high}. 
%
Incoherence can also seen as a inclusion criteria for a unit $n$ to be included in the donor set $\mathcal{I}$.  
%
Lemma 2 in \cite{negahban2012learning} shows that the Assumption \ref{ass:incoherence} is satisfied with high probability if $\Pi_u$ is chosen uniformly at random and grows as $\omega(s^2p)$. 
%
If Assumption \ref{ass:incoherence} does not hold, then the Lasso may not estimate $\balpha_u$ accurately, and alternative horizontal regression algorithms may be required instead. 
%
Assumption \ref{ass:balanced_spectrum} requires that the non-zero singular values of $\E[\bY_{\mathcal{I}}^{(\Pi_n)} ~ | ~ \mathcal{A}]$ are well-balanced. 
%
This assumption is standard when studying PCR \cite{agarwal2019robustness,agarwal2020synthetic}, and within the econometrics literature \cite{bai2021matrix,fan2018eigenvector}. 
%
It can also be empirically validated by plotting the spectrum of $\hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n)}]$; if the singular spectrum of $\hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n)}]$ displays a natural elbow point, then Assumption \ref{ass:balanced_spectrum} is likely to hold. 
%
Assumption \ref{ass:rowspace_inclusion} is also commonly made when analyzing PCR \cite{agarwal2020principal,agarwal2020synthetic,agarwal2021causal}.
%
It can be thought of as a ``causal transportability'' condition from the model learnt using $\Pi_n$ to the interventions $\pi \in \Pi \setminus \Pi_n$. 
%
That is, subspace inclusion allows us to generalize well, and accurately estimate $\E[Y_n^{(\pi)} ~ | ~ \mathcal{A} ]$ using $\langle \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n)}], \hat{\bw}^n \rangle$. 
%
In Section \ref{sec:experimental_design}, we propose a simple experimental design mechanism that ensures that Assumptions \ref{ass:incoherence}, \ref{ass:balanced_spectrum}, \ref{ass:rowspace_inclusion} (and Assumption  \ref{ass:donor_set_identification}), i.e., the key conditions for \method~to work, hold with high probability. 
%As we show in Section \ref{sec:experimental_design}, subspace inclusion holds with high probability if $|\Pi_n|$ is chosen uniformly and independently at random from $\Pi$ and has size $\omega(r\log(|\mathcal{I}|))$.
\vspace{-2mm}

\subsection{Finite Sample Consistency}\label{subsec:finite_sample_consistency}
\vspace{-2mm}
%
The following result establishes finite-sample consistency of \method. 
%
Without loss of generality, we will focus on estimating the pair of quantities $(\E[Y_u^{(\pi)}],\E[Y_n^{(\pi)}])$ for a given donor unit $u \in \mathcal{I}$, and non-donor unit $n \in [N] \setminus \mathcal{I}$ under treatment assignment $\pi \in \Pi$.
%
To simplify notation, we will use $O_p$ notation:
%
for any sequence of random vectors $X_n$, $X_n$ = $O_p(\gamma_n)$ if, for any $\epsilon > 0$, there exists constants $c_\epsilon$ and $n_\epsilon$ such that $\mathbb{P}(\lVert X_n \rVert_2 \geq c_\epsilon\gamma_n) \leq \epsilon$ for every $n \geq n_\epsilon$. 
%
Additionally, we absorb dependencies on $\sigma$ into $O_p$.
%
For simplicity, we also define $\tilde{O_p}(\gamma_n)$ which suppresses  logarithmic terms. 
%

\begin{theorem} [Finite Sample Consistency of \method]
\label{thm:potential_outcome_convergence_rate}
Conditioned on $\mathcal{A}$, let Assumptions \ref{ass:observation_model}, \ref{ass:selection_on_fourier}, \ref{ass:donor_set_identification}, \ref{ass:boundedness_potential_outcome}, \ref{ass:subgaussian_noise}, and \ref{ass:incoherence} hold. Then, the following statements hold. 
\begin{itemize}
    \item [(a)] For any donor unit-combination pair $(u,\pi)$, let the Lasso regularization parameter satisfy $\lambda_u = \Omega(\sqrt{\frac{p}{|\Pi_u|}})$, then we have that
        $$
            |\hat{\E}[Y_u^{(\pi)}] - \E[Y_{u}^{(\pi)}]| = O_p\left(s\sqrt{\frac{p}{|\Pi_u|}}\right).
        $$
    \item [(b)] Additionally, let Assumptions \ref{ass:balanced_spectrum}, and \ref{ass:rowspace_inclusion} hold. Then, for any non-donor unit-combination pair $(n,\pi)$ where $n \in [N] \setminus \mathcal{I}$, if $\kappa_n = \text{rank}(\E[\bY_{\mathcal{I}}^{(\Pi_n)}]) \coloneqq r_{n}$, and $ \min_{u \in \mathcal{I}} |\Pi_u| \coloneqq M = \omega(s^2p)$, we have that,
        $$
            \left |\hat{\E}[Y_n^{(\pi)}] - \E[Y_{n}^{(\pi)}]\right|  = \Tilde{O_p}\left(r^{3/2}_n\left[\frac{1}{\min\{\sqrt{|\Pi_n|},\sqrt{|\mathcal{I}|}\}} + s\sqrt{\frac{{p}}{{M}}}  \right]\right).
        $$
\end{itemize}

\end{theorem}
\vspace{-2.5mm}
%
Establishing Theorem \ref{thm:potential_outcome_convergence_rate} requires a novel analysis of error-in-variables (EIV) linear regression.
%
Specifically, the general EIV linear model is as follows: $Y = \bX \beta + \epsilon$, $\mathbf{Z} = \bX + \mathbf{H}$, where $Y$ and $\mathbf{Z}$ are observed.
%
In our case, $Y = \bY_{\Pi_n}$, $\bX = \E[\bY_{\mathcal{I}}^{(\Pi_n)}]$, $\beta = \bw^n$ , $\bZ = \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n)}]$, and $\mathbf{H}$ is the error arising in estimating $\E[\bY_{\mathcal{I}}^{(\Pi_n)}]$ via the Lasso.
%
Typically one assumes that $\mathbf{H}$ is is a matrix of independent sub-gaussian noise. 
%
Our analysis requires a novel worst-case analysis of $\mathbf{H}$ (due to the 2-step regression of Lasso and then PCR), in which each entry of is  $\mathbf{H}$ simply bounded.

%Previous works assume that $\bH$ is is a matrix of independent sub-gaussian noise. Our analysis requires a worst-case analysis of H (due to the 2-step regression of Lasso and then PCR), which each entry of is H simply bounded. } 
%$\bZ = \bX + \bH$, where $Y$ and $\bZ$ are observed. }


%in our setting, the covariate matrix used in PCR (i.e., $\hat{\E}[Y_{\mathcal{I}}^{(\Pi_n)}]$) is corrupted by bounded noise that arises from estimating potential outcomes via the Lasso for the donor set. This differs from previous work in which the covariate matrix is corrupted by independent sub-gaussian noise. }

Next, we describe the conditions required on $|\Pi_n|$,$|\mathcal{I}|$, $M$, for \method~to consistently estimate $(\E[Y_u^{(\pi)}], \ \E[Y_n^{(\pi)}])$. 
%
Specifically, if $\min\{|\Pi_n|,|\mathcal{I}|\} = \omega(r^3_n)$ and $M = \omega(r^3_ns^2p)$, then $\max\left(|\hat{\E}[Y_u^{(\pi)}] - \E[Y_{u}^{(\pi)}]|, \\ |\hat{\E}[Y_n^{(\pi)}] - \E[Y_{n}^{(\pi)}]|\right) =\tilde{o}_p(1)$.
%
Next, we present a corollary that discusses how quickly the parameters $r_n$, $s$, and $p$ can grow with the number of observations $|\Pi_n|$, $\mathcal{I}$, and $M$.


\begin{corollary}\label{cor:potential_outcome_convergence_rate_simplified}
%
With the set-up of Theorem \ref{thm:potential_outcome_convergence_rate}, if the following conditions hold: $r_n = o(\min\{|\Pi_n|,|\mathcal{I}|\}^{1/3})$, and $s = o\left(\sqrt{\frac{M}{pr^3_n}} \right)$, then 
$
\max\left(|\hat{\E}[Y_u^{(\pi)}] - \E[Y_{u}^{(\pi)}]|, \\ \ |\hat{\E}[Y_n^{(\pi)}] - \E[Y_{n}^{(\pi)}]|\right) =\tilde{o}_p(1) 
$ as $|\Pi_n|, |\mathcal{I}|, $M$ \to \infty$. 
%
\end{corollary}

\vspace{-1.5mm}
%
\noindent Corollary \ref{cor:potential_outcome_convergence_rate_simplified} quantifies how $s, r_n$ can scale with the number of observations to achieve consistency. 
%
That is, Corollary \ref{cor:potential_outcome_convergence_rate_simplified} reflects the maximum ``complexity'' allowed for a given sample size. 

\subsection{Finite-Sample Consistency of CART}
\label{subsec:CART_finite_sample}

\noindent As discussed in Section \ref{sec:estimator_descripton}, \method~allows for any ML algorithm to be used for horizontal regression. 
%
In this section, we present theoretical results when the horizontal regression is done via CART. 
%
We show that when the potential outcome function is a $k$-Junta (see equation \eqref{eq:k_junta} for the definition), CART is able to achieve stronger sample complexity guarantees than the Lasso. 
%
We refer the reader to Appendix \ref{sec:CART_horizontal_regression} for a description of the CART algorithm.
%
Our CART-based horizontal regression procedure consists of the following two steps. 


\noindent \textbf{Step 1: Feature Identification.} For each donor unit $u \in \mathcal{I}$, divide the observed interventions $\Pi_u$ equally into two sets $\Pi^{a}_u$ and $\Pi^{b}_u$. Fit a CART model $\mathcal{\hat{T}}$ on the dataset $\mathcal{D}^a_u = [\{\bv(\pi),Y_{u\pi}\}: \pi \in \Pi^a_u]$. Let $\hat{K}_u = \{\bv(\pi)_j : \bv(\pi)_j$ $\in \mathcal{\hat{T}}\}$ denote every feature that the CART splits on. 

\noindent \textbf{Step 2: Estimation.} For every subset $S \subset \hat{K}_u$, compute $\hat{\alpha}_{u,S} = \frac{1}{|\Pi^b_u|}\sum_{\pi \in \Pi^b_u }Y_{u\pi}\chi^{\pi}_{S}$. We then estimate our target causal parameter as follows: $\hat{\E}[Y_u^{(\pi)}] = \sum_{S \in \hat{K}_u}\hat{\alpha}_{u,S}\chi^{\pi}_{S}$.

\noindent CART is able to take advantage of the $k$-Junta structure of the potential outcomes by first performing feature selection (i.e., learning the relevant feature set $\hat{K}_u$), before estimating the Fourier coefficient for each relevant subset.
%
In contrast, Lasso estimates the Fourier coefficient of all $2^p$ subsets simultaneously. 
%

Next, we present our theoretical results that establishes CART exploits this $k$-Junta structure to provide better sample complexity guarantees than the Lasso.
%
Specifically, we present an informal theorem for the horizontal regression finite sample error when the horizontal regression is done via CART.  
%
The formal result (Theorem \ref{thm:CART_convergence_rate}) can be found in Appendix \ref{supp:CART_finite_sample}. 

\begin{theorem} [Informal]
\label{thm:informal_CART_potential_outcome_convergence_rate}
For a given donor unit $u$, suppose $\E[Y_u^{(\pi)}]$ is a $k$-Junta, then, if the horizontal regression is done via CART, we have
        $
            |\hat{\E}[Y_u^{(\pi)}] - \E[Y_{u}^{(\pi)}]| = \Tilde{O}_p\left(\frac{s}{\sqrt{|\Pi_u|}}\right).
       $
\end{theorem}
%
Compared to the Lasso horizontal regression error (see Theorem \ref{thm:potential_outcome_convergence_rate} (a)), CART removes an additional factor of $p$ by exploiting the $k$-Junta structure. 
%
As a result, it can be verified that CART also removes a factor of $p$ for the vertical regression error (see Theorem \ref{thm:potential_outcome_convergence_rate} (b)). 
%
Next, we describe the conditions required for $\Pi_n$, $M$ to consistently estimate $(\E[Y_u^{(\pi)}], \ \E[Y_n^{(\pi)}])$ for a given donor unit $u$, non-donor unit $n$, and combination $\pi$ with \method~when the horizontal regression is done via CART.
%
Given this assumption, it can be verified that if $\min\{|\Pi_n|,|\mathcal{I}|\} = \omega(r^3_n)$, and $M = \omega(r^3_ns^2)$, then $\max\left(|\hat{\E}[Y_u^{(\pi)}] - \E[Y_{u}^{(\pi)}]|, \ |\hat{\E}[Y_n^{(\pi)}] - \E[Y_{n}^{(\pi)}]|\right) =\tilde{o}_p(1)$.
%
That is, CART reduces the number of required observations for donor units by a factor of $p$.



%\begin{corollary}
%\label{cor:potential_outcome_convergence_rate_CART}
%
%Let the set-up of Theorems \ref{thm:potential_outcome_convergence_rate}, \ref{thm:CART_convergence_rate}, and condition (a) of Corollary \ref{cor:potential_outcome_convergence_rate_simplified} hold. 
%
%Then, if $s =  o\left(\sqrt{M/(\max\{|\Pi_n|,|\mathcal{I}|\}})\right)$, 
%$\max\left(|\hat{\E}[Y_u^{(\pi)}] - \E[Y_{u}^{(\pi)}]|, \ |\hat{\E}[Y_n^{(\pi)}] - \E[Y_{n}^{(\pi)}]|\right) =\tilde{o}_p(1)$
%
%\end{corollary} 
%\vspace{-2mm}
%
%\noindent Corollary \ref{cor:potential_outcome_convergence_rate_CART} 
%shows CART can achieve consistency while allowing the sparsity $s$ to scale more quickly (i.e., by a factor of $p$) than the Lasso. 
%
%That is, CART exploits the additional regularity conditions placed on the potential outcomes to achieve consistency with $M = \omega(r_n^4s^2)$ samples. 
%
%As discussed above, the superior sample complexity of CART arises from the fact that it identifies the relevant feature subset before estimating the Fourier coefficient.
%

%shows CART exploits the additional regularity conditions placed on the potential outcomes to allow the sparsity $s$ to scale more quickly (i.e., by a factor of $p$) while maintaining consistency. 



\subsection{Sample Complexity}
\label{subsec:sample_complexity_synth_combo}
\vspace{-2.5mm}
We discuss the sample complexity of \method~to estimate all $N \times 2^p$ causal parameters, and compare it to that of other methods.
%
To ease our discussion, we will ignore dependence on logarithmic factors, and assume that $|\Pi_n| = |\mathcal{I}|$.
%
Further, we remind the reader that we denote $\min_{u \in \mathcal{I}} \coloneqq M$. 
%
We also assume that the horizontal regression is done via the Lasso. 

%
Even if potential outcomes $Y_n^{(\pi)}$ were observed for all unit-combination pairs, consistently estimating $\E[\bY_N^{(\Pi)}]$ is not trivial. 
%
This is because, we only get to observe a single and noisy version $Y_{n\pi} = \langle \balpha_n, \bchi^{\pi} \rangle + \epsilon_n^{\pi}$. 
%
Hypothetically, if we observe $K$ independent samples of $Y_{n\pi}$ for a given $(n,\pi)$, denoted by $Y^{1}_{n\pi}, \ldots, Y^{K}_{n\pi}$, the maximum likelihood estimator would be the empirical average $\frac{1}{K}\sum^K_{i=1}Y^{i}_{n\pi}$. 
%
The empirical average would concentrate around $\E[Y_n^{(\pi)}]$ at a rate $O(1/\sqrt{K})$ and hence would require $K = \Omega(\delta^{-2})$ samples to estimate $\E[Y_n^{(\pi)}]$ within error $O(\delta)$. 
%
Therefore, this naive (unimplementable) solution would require $N \times 2^p \times \delta^{-2}$ observations to estimate $\E[\bY_N^{(\Pi)}]$. 
%

On the other hand, \method~produces consistent estimates of the potential outcome despite being given {\em at most only a single noisy sample} of each potential outcome. 
%
As our discussion after Theorem \ref{thm:potential_outcome_convergence_rate} shows, 
$|\mathcal{I}| \times r^3s^2p/\delta^2$ observations for the donor set, and $(N - |\mathcal{I}|) \times r^3/\delta^2$ observations for the non-donor units to achieve an estimation error of $O(\delta)$ for all $N \times 2^p$ causal parameters. 
%
Assuming $|\Pi_n| = |\mathcal{I}|$, this implies that the number of observations required to achieve an estimation error of $O(\delta)$ for all pairs $(n,\pi)$ via \method~scales as $O\left(\text{poly}(r/\delta) \times \left(N + s^2p \right) \right)$.


\vspace{2mm}
\noindent \textbf{Sample Complexity Comparison to Other Methods.}  

\noindent \emph{Horizontal regression:} An alternative algorithm would be to learn an individual model for each unit $n \in [N]$. 
%
That is, run a separate horizontal regression via the Lasso for every unit.
%
This alternative algorithm has sample complexity that scales at least as $O(N \times s^2p/\delta^2)$  rather than $O\left(\text{poly}(r)/\delta^4  \times \left(N + s^2p \right) \right)$ required by \method.  
%
It suffers because it does not utilize any structure across units (i.e., the low-rank property of $\mathcal{A}$), whereas \method~captures the similarity between units via PCR. 
%

\vspace{1mm}
\noindent \emph{Matrix completion:} \method~can be thought of as a matrix completion method; estimating $\E[Y_n^{(\pi)}]$ is equivalent to imputing $(n,\pi)$-th entry of the observation matrix $\bY \in \{\mathbb{R} \cup \star\}^{N \times 2^p}$, where recall $\star$ denotes an unobserved unit-combination outcome. 
%
Under the low-rank property (Assumption \ref{ass:observation_model}(b)) and various models of missingness (i.e., observation patterns), recent works on matrix completion \cite{candes2010matrix,ma2019missing,agarwal2021causalmatrix} (see Section \ref{sec:related_work} for an overview) have established that estimating $\E[Y_n^{(\pi)}]$ to an accuracy $O(\delta)$ requires at least $O\left(\text{poly}(r/\delta) \times \left(N + 2^p \right)\right)$ samples.
%
This is because matrix completion techniques do not leverage the sparsity of $\balpha_n$.
%leverage additional structural information such as the Fourier expansion of Boolean functions and the resulting sparsity in $\balpha_n$.
%
Moreover, matrix completion results typically report error in the Frobenius norm, whereas we give entry-wise guarantees. 
%
This leads to an extra factor of $s$ in our analysis as it requires proving convergence for $\lVert \hat{\balpha_n} - \balpha_n \rVert_{1}$ rather than $\lVert \hat{\balpha_n} - \balpha_n \rVert_{2}$. 
%
% Hence, \method~combines the best of both approaches by leveraging both the structure of the potential outcomes \emph{and} the similarity across units. 

\vspace{2mm}
\noindent \textbf{Natural Lower Bound on Sample Complexity.} We provide an informal discussion on the lower bound sample-complexity to estimate all $N \times 2^p$ potential outcomes. 
%
As established in Lemma \ref{lem:number_nonzeros}, $\mathcal{A}$ has at most $rs$ non-zero columns. 
%
Counting the parameters in the singular value decomposition of $\mathcal{A}$, only $r\times (N + rs)$ free parameters are required to be estimated. 
%
Hence, a natural lower bound on the sample complexity scales as $O(Nr + r^2s)$.  
%
Hence, \method~is only sub-optimal by a factor (ignoring logarithmic factors) of $sp$ and $\text{poly}(r)$.  
%
As discussed earlier, an additional factor of $s$ can be removed if we focus on deriving Frobenius norm error bounds.
%
Further, the use of non-linear methods such as CART can remove the factor of $p$ (Theorem \ref{thm:informal_CART_potential_outcome_convergence_rate}) under stronger assumptions on the potential outcomes such as when $\E[Y_n^{(\pi)}]$ is a $k$-Junta that satisfies regularity conditions. 
%
It remains interesting future work to derive estimation procedures that are able to achieve this lower bound.


%
%To simplify the discussion, we assume that $\min\{|\Pi_n|,|\mathcal{I}|\} = \mathcal{|I|}$. 
%
%This condition can be enforced in practice by simply picking a subset of donor units such that $|\mathcal{I}| \leq |\Pi_n|$ when performing PCR (i.e., step 2 of \method).


%Next, we present a corollary analogous to Corollary \ref{cor:potential_outcome_convergence_rate_simplified} that discusses how quickly 
%that assumes the horizontal regression is done via CART instead. 



%present the additional assumptions required on the potential outcomes for finite-sample consistency of \method~when using CART instead of Lasso. 
%
%We only present an informal discussion of these assumptions, and leave the precise formulation to Appendix \textcolor{red}{H}.  

% how quickly the parameters $r_n,s,p$ are allowed to grow with the number of observations $|\Pi_n|$, and $M$ for \method~with CART to achieve consistency. 

% o\left(\sqrt{M/(p\max\{|\Pi_n|,|\mathcal{I}|\}})\right) $




%for estimating our target causal parameter via \method.  
%
%{\color{red} Specifically, we establish a corollary analogous to Corollary \ref{cor:potential_outcome_convergence_rate_simplified} that quantifies the maximum complexity (as measured by $r_n,s,p$) allowed by CART for a given sample size. 
%
%Before presenting the corollary, we provide an informal discussion of the assumptions imposed on the potential outcomes $\E[Y_n^{(\pi)}]$ required for CART to achieve finite-sample consistency. 
%
%We assume: (i) $\E[Y_n^{(\pi)}]$ is a $k$-Junta as discussed above, (ii) $\E[Y_n^{(\pi)}]$ satisfies a ``sub-modularity'' condition which is necessary for greedy-tree algorithms such as CART to achieve consistency (see Definition \ref{def:strong_partition_sparsity} for an exact characterization of this sub-modularity condition), and (iii) the combinations of donor units are observed uniformly at random. 
%
%Given this discussion on the required assumptions, we present our theoretical result as follows.}

%To satisfy linear span inclusion (Assumption \ref{ass:donor_set_identification} (b)), and the necessary conditions for PCR (i.e., Assumption \ref{ass:rowspace_inclusion}), we require that donor set has size $|\mathcal{I}| = \omega(r)$. 
%Indeed, we verify in our experimental design mechanism in Section \ref{sec:experimental_design} that uniformly choosing a donor set of size $|\mathcal{I}| = O(r)$ satisfies these assumptions.

%Hence, at most $N \times r^4/\delta^4$ + $|\mathcal{I}| \times r^4s^2p/\delta^2$ observations are required to estimate $\E[Y_n^{(\pi)}]$ with error $O(\delta)$ for all pairs $(n,\pi)$. 
%
%Of course, this is assuming that the key assumptions (see Section \ref{subsec:finite_sample_analysis_assumptions}) are satisfied. 
%
%Hence, we have that the number of observations required to achieve an estimation error of $O(\delta)$ scales as $O\left(\text{poly}(r)/\delta^4 \times \left(N + s^2p \right) \right)$. 
%

==> archive/finite_sample_consistency_tightened_2.tex <==
\section{Proof of Theorem \ref{thm:potential_outcome_convergence_rate}}

\subsection{Proof of Theorem  \ref{thm:potential_outcome_convergence_rate} (a)}
We have that 
\label{subsec:horizontal_regression_theorem_proof}
\begin{align} 
     \hat{\E}[Y_u^{(\pi)}] - \E[Y_{u}^{(\pi)}] & = \langle  \hat{\balpha}^u, \bchi^{\pi} \rangle - \langle  \balpha_u, \bchi^{\pi} \rangle \nonumber\\
     & = \langle  \hat{\balpha}_u - \balpha_u, \bchi^{\pi} \rangle \nonumber \\
     & \leq \lVert \hat{\balpha}_u - \balpha_u \rVert_1 \lVert \bchi^{\pi} \rVert_{\infty} \nonumber \\ 
     & = \lVert \hat{\balpha}_u - \balpha_u \rVert_1 \label{eq:lasso_proof_holder_inequality}
\end{align}

\noindent To finish the proof, we quote the following Theorem which we adapt to our notation. 

\begin{theorem}[Theorem 2.18 in \cite{rigollet2015high}] 
\label{thm:rigollet_lasso_high_prob_bound}
Fix the number of samples $n \geq 2$. Assume that the linear model $Y = \bX\theta^* + \epsilon$, where $\bX \in \mathbb{R}^{n \times d}$ and $\epsilon$ is a sub-gaussian random variable with noise variance $\sigma^2$. Moreover, assume that $\lVert \theta^* \rVert_0 \leq k$, and that 
$\bX$ satisfies the incoherence condition (Assumption \ref{ass:incoherence}) with parameter $k$. Then, the lasso estimator $\hat{\theta}^L$ with regularization parameter defined by 
\begin{equation*}
    2\tau = 8\sigma\sqrt{\log(2d)/n} +  8\sigma\sqrt{\log(1/\delta)/n}
\end{equation*}
satisfies 
\begin{equation}
    \lVert \theta^* - \hat{\theta}^L \rVert^2_2 \leq k\sigma^2\frac{\log(2d/\delta)}{n}
\end{equation}
with probability at least $1 - \delta$. 
\end{theorem}
Further, as in established in the proof of Theorem 2.18 in \cite{rigollet2015high}, $\lVert \theta^* - \hat{\theta}^L \rVert_1 \leq \sqrt{k} \lVert \theta^* - \hat{\theta}^L \rVert_2$. Note that the set-up of Theorem \ref{thm:rigollet_lasso_high_prob_bound} holds in our setting with the following notational changes: $Y = \bY_{\Pi_u}$, $\bX = \bchi(\Pi_u)$, $\theta^* = \balpha_u$, $\hat{\theta}^L = \hat{\balpha}_u$,  $k = s$ as well as our assumptions on the regularization parameter $\lambda_u$ and that $\bepsilon_u^{\pi}$ is sub-gaussian (Assumption \ref{ass:subgaussian_noise}). Applying Theorem \ref{thm:rigollet_lasso_high_prob_bound} gives us
\begin{equation*}
    \lVert \hat{\balpha}_u - \balpha_u \rVert_1 = O_p \left(s \sqrt{\frac{p}{|\Pi_u|}}\right)
\end{equation*}
Substituting this bound into \eqref{eq:lasso_proof_holder_inequality} yields the claimed result. 


%\section{Lasso Horizontal Regression Analysis}
%\label{sec:Lasso_finite_sample_analysis}

%\begin{proposition} 
%\label{prop:Lasso_convergence_rate} 
%Let Assumptions \ref{ass:observation_model}, \ref{ass:subgaussian_noise}, and \ref{ass:incoherence} hold. Then, conditioned on $\mathcal{A}$, we have
%\begin{equation}
%\label{eq:Lasso_convergence_rate}
% \hat{\E}[Y_u^{(\pi)}] - \E[Y_u^{(\pi)}] = O_p\left(\sqrt{\frac{s^2p}{|\Pi_u|}} ~ \bigg | ~ \mathcal{A} \right) 
%\end{equation}
%for any donor unit $u \in\mathcal{I}$ and $\pi \in \Pi$
%\end{proposition}



\subsection{Proof of Theorem  \ref{thm:potential_outcome_convergence_rate} (b)}
For any matrix $\mathbf{A}$ with orthonormal columns, let $\mathcal{P}_{A} = \mathbf{A}\mathbf{A}^T$ denote the projection matrix on the subspace spanned by the columns of $\mathbf{A}$. Define $\Tilde{\bw}^n = \mathcal{P}_{V_{\mathcal{I}}^{(\Pi_n)}}\bw^n$, where $\bV_{\mathcal{I}}^{(\Pi_n)}$ are the right singular vectors of $\E[\bY_{\mathcal{I}}^{(\Pi_n)}]$. Let $\Delta^n_w = \hat{\bw}^n - \Tilde{\bw}^n \in \R^{|\mathcal{I}|}$, and $\Delta_{\mathcal{I}}^{\pi} = \hat{\E}[\bY_{\mathcal{I}}^{(\pi)}] - \E[\bY_{\mathcal{I}}^{(\pi)}] \in \R^{|\mathcal{I}|}$. Denote $\Delta_E = \max_{u \in \mathcal{I}, \pi \in \Pi} \left |\hat{\E}[Y_u^{(\pi)}] - \E[Y_{u}^{(\pi)}] \right |$. Throughout the proof, we use $C$ to refer to constants that might change from line to line. Additionally, we use $\vee$ to denote maximum. In order to proceed, we first state the following result,  
\begin{lemma} 
\label{lem:w_tilde_transfer_outcomes}
Let the set-up of Theorem \ref{thm:potential_outcome_convergence_rate} hold. Then, we have 
\begin{equation*}
    \E[Y_{n}^{(\pi)}] =  \langle \E[\bY_{\mathcal{I}}^{(\pi)}], \Tilde{\bw}^n \rangle
\end{equation*}
\end{lemma}

\noindent Using Lemma \ref{lem:w_tilde_transfer_outcomes}, and the notation established above, we have
\begin{align}
     \left |\hat{\E}[Y_n^{(\pi)}] - \E[Y_{n}^{(\pi)}]\right| & = \left| \langle \hat{\E}[\bY_{\mathcal{I}}^{(\pi)}], \hat{\bw}^n \rangle - \langle \E[\bY_{\mathcal{I}}^{(\pi)}], \Tilde{\bw}^n \rangle \right| \nonumber \\
     & \leq \left| \langle \Delta_{\mathcal{I}}^{\pi}, \Tilde{\bw}^n \rangle \right| +  \left| \langle \E[\bY_{\mathcal{I}}^{(\pi)}] ,\Delta^n_w   \rangle \right| + \left| \langle \Delta^n_w, \Delta_{\mathcal{I}}^{\pi} \rangle \right| \label{eq:three_term_bound_pre_projection}
\end{align}
%From Assumption \ref{ass:rowspace_inclusion}, it follows that $\E[\bY_{\mathcal{I}}^{(\pi)}] = \mathcal{P}_{V_{\mathcal{I}}^{(\Pi_n)}} \E[\bY_{\mathcal{I}}^{(\pi)}]  $ , where $\bV_{\mathcal{I}}^{(\Pi_n)}$ are the right singular vectors of $\E[\bY_{\mathcal{I}}^{(\Pi_n)}]$. Using this in \eqref{eq:three_term_bound_pre_projection} gives us
%\begin{equation}
 %\label{eq:three_term_bound_post_projection}
%   \left |\hat{\E}[Y_n^{(\pi)}] - \E[Y_{n}^{(\pi)}]\right| \leq  \left| \langle \Delta_{\mathcal{I}}^{\pi}, \Tilde{\bw}^n \rangle \right| +  \left| \langle \E[\bY_{\mathcal{I}}^{(\pi)}] ,\mathcal{P}_{V_{\mathcal{I}}^{(\Pi_n)}}\Delta^n_w   \rangle \right| + \left| \langle \Delta^n_w, \Delta_{\mathcal{I}}^{\pi} \rangle \right|
%\end{equation}
Below, we bound the three terms on the right-hand-side of \eqref{eq:three_term_bound_pre_projection} separately. Before we bound each term, we state a Lemma that will be useful to help us establish the results. 

\begin{lemma} 
\label{lem:l1_bound_w_tilde}
Let Assumptions \ref{ass:observation_model}, \ref{ass:donor_set_identification}, \ref{ass:boundedness_potential_outcome}, and \ref{ass:balanced_spectrum} hold. Then, $\lVert \tilde{\bw}^n \rVert_2 \leq C\sqrt{\frac{r_n}{|\mathcal{I}|}}$
\end{lemma}


\noindent \emph{Bounding Term 1.} By Holder's inequality and Lemma \ref{lem:l1_bound_w_tilde}, we have that 
\begin{equation}
\label{eq:Term1_Op_bound}
    \left| \langle \Delta_{\mathcal{I}}^{\pi}, \Tilde{\bw}^n \rangle \right| \leq \lVert \Tilde{\bw}^n \rVert_1 \lVert \Delta_{\mathcal{I}}^{\pi} \rVert_\infty \leq \lVert \Tilde{\bw}^n \rVert_1 \Delta_E \leq  \sqrt{|\mathcal{I}|}\lVert \Tilde{\bw}^n \rVert_2 \Delta_E \leq C\sqrt{r_n}\Delta_E
\end{equation}
\noindent This concludes the analysis for the first term. \\ 

\noindent \emph{Bounding Term 2}. By Cauchy-Schwarz and Assumption \ref{ass:boundedness_potential_outcome} we have,  
\begin{align}
    \left| \langle \E[\bY_{\mathcal{I}}^{(\pi)}] , \Delta^n_w \rangle \right |  \leq \lVert \E[\bY_{\mathcal{I}}^{(\pi)}] \rVert_2 \lVert \Delta^n_w  \rVert_2  \leq \sqrt{|\mathcal{I}|} \lVert \Delta^n_w  \rVert_2 \label{eq:term2_cauchy_schwarz}
\end{align}
\noindent We now state a proposition that will help us conclude our bound of Term 2. The proof is given in Appendix \ref{subsec:pcr_proofs}. 


\begin{proposition}
\label{prop:pcr_convergence_rate} Let the set-up of Theorem \ref{thm:potential_outcome_convergence_rate} hold. Then, conditioned on $\mathcal{A}$, we have 
\begin{equation}
    \hat{\bw}^n - \Tilde{\bw}^n=  {O}_p \left(\log^{3}(|\Pi_n||\mathcal{I}|)r_n \lVert \Tilde{\bw}^{n} \rVert_2 \left[\frac{1 }{\min\{\sqrt{|\Pi_n|},\sqrt{|\mathcal{I}|\}}}  + \Delta_E \right] \right) 
\end{equation}
\end{proposition}

\noindent Substituting the result of Lemma \ref{lem:l1_bound_w_tilde}, and Proposition \ref{prop:pcr_convergence_rate} into \eqref{eq:term2_cauchy_schwarz}, we have the following bound for term 2. 
\begin{equation}
\label{eq:Term2_Op_bound}
     \left| \langle \E[\bY_{\mathcal{I}}^{(\pi)}] , \Delta^n_w \rangle \right | = O_p\left(\log^{3}(|\Pi_n||\mathcal{I}|)r^{3/2}_n  \left[\frac{1 }{\min\{\sqrt{|\Pi_n|},\sqrt{|\mathcal{I}|\}}}  + \Delta_E \right] \right)
\end{equation}

\noindent \emph{Bounding Term 3.} By Holder's inequality,  we have that
\begin{align}
    \left| \langle \Delta^n_w, \Delta_{\mathcal{I}}^{\pi} \rangle \right| & \leq \lVert \Delta^n_w \rVert_2 \lVert \Delta_{\mathcal{I}}^{\pi} \rVert_2 \nonumber \\
    & \leq \sqrt{|\mathcal{I}|} \lVert \Delta^n_w \rVert_2 \lVert \Delta_{\mathcal{I}}^{\pi} \rVert_\infty \nonumber \\
    & \leq  \sqrt{|\mathcal{I}|} \Delta_E \lVert \Delta^n_w \rVert_2 \label{eq:term3_holder} 
\end{align}
\noindent Substituting the result of  Lemma \ref{lem:l1_bound_w_tilde}, and Proposition \ref{prop:pcr_convergence_rate} into \eqref{eq:term3_holder} gives us the following bound for term 3, 

\begin{equation}
\label{eq:Term3_Op_bound}
     \left| \langle \Delta^n_w, \Delta_{\mathcal{I}}^{\pi} \rangle \right| = O_p \left(\log^{3}(|\Pi_n||\mathcal{I}|)r^{3/2}_n \left[\frac{\Delta_E  }{\min\{\sqrt{|\Pi_n|},\sqrt{|\mathcal{I}|\}}}  + \Delta^2_E \right] \right)
\end{equation}

\noindent \emph{Collecting Terms.} Combining equations \eqref{eq:Term1_Op_bound}, \eqref{eq:Term2_Op_bound}, \eqref{eq:Term3_Op_bound} gives us
\begin{equation}
\label{eq:collecting_terms}
\begin{split}
&\left |\hat{\E}[Y_n^{(\pi)}] - \E[Y_{n}^{(\pi)}]\right|   
\\ &= O_p\left(\log^{3}(|\Pi_n||\mathcal{I}|) r_n^{3/2} (1 \vee \Delta_E) \left[\frac{1}{\min\{\sqrt{|\Pi_n|},\sqrt{|\mathcal{I}|\}}}  + \Delta_E \right] \right)  
\end{split}
\end{equation} 

\noindent By Theorem \ref{thm:potential_outcome_convergence_rate} (a), we have that 
\begin{equation}
\label{eq:delta_E_subsitution}
    \Delta_E = \max_{u \in \mathcal{I}} \ O_p \left(s\sqrt{\frac{p}{|\Pi_u|}}\right) = O_p \left(s\sqrt{\frac{p}{M}}\right)
\end{equation}
\noindent where we remind the reader that $M = \min_{u \in \mathcal{I}} |\Pi_u|$. Substituting \eqref{eq:delta_E_subsitution} into \eqref{eq:collecting_terms}, and simplifying, then we get 
\begin{equation}
\label{eq:collecting_terms_simplified_1}
\begin{split}
\left |\hat{\E}[Y_n^{(\pi)}] - \E[Y_{n}^{(\pi)}]\right|  = O_p\left(\log^{3}(|\Pi_n||\mathcal{I}|)r^{3/2}_n\left(\sqrt{\frac{s^2p}{M}} \vee  1 \right) \left[\frac{1}{\min\{\sqrt{|\Pi_n|},\sqrt{|\mathcal{I}|\}}}  + \sqrt{\frac{s^2p}{M}} \right]  \right)  
\end{split}
\end{equation}


\noindent Substituting our assumption that $M \coloneqq \omega(s^2p)$, we get 
\begin{equation}
\label{eq:collecting_terms_simplified_log}
\begin{split}
\left |\hat{\E}[Y_n^{(\pi)}] - \E[Y_{n}^{(\pi)}]\right|  = O_p\left(\log^{3}(|\Pi_n||\mathcal{I}|)r^{3/2}_n \left[\frac{1}{\min\{\sqrt{|\Pi_n|},\sqrt{|\mathcal{I}|\}}}  + \sqrt{\frac{s^2p}{M}} \right]  \right)  
\end{split}
\end{equation}
\noindent Finally, absorbing the logarithmic factors, we get the claimed result, 
\begin{equation}
\label{eq:collecting_terms_simplified}
\begin{split}
\left |\hat{\E}[Y_n^{(\pi)}] - \E[Y_{n}^{(\pi)}]\right|  = O_p\left(r^{3/2}_n \left[\frac{1}{\min\{\sqrt{|\Pi_n|},\sqrt{|\mathcal{I}|\}}}  + \sqrt{\frac{s^2p}{M}} \right]  \right)  
\end{split}
\end{equation}


%and our assumption that $M = \omega(r^2_ns^2p)$


%\sqrt{\frac{s^2p}{M}} r_n^{2}\left[\frac{1}{\min\{\sqrt{|\Pi_n|},\sqrt{|\mathcal{I}|\}}}  +  \sqrt{\frac{s^2p|\mathcal{I}|}{M}} \right]  + \frac{r_n}{|\Pi_n|^{1/4}}  \right)  
%\end{split} %\left( \right)
%We now state a lemma that will help us simplify the result, and conclude the proof.
%The proof of this lemma can be found in Appendix \ref{subsec:proof_of_l1_bound_w_tilde}.
%Substituting the result of Lemma \ref{lem:l1_bound_w_tilde} and Theorem \ref{thm:potential_outcome_convergence_rate} (a)  into \eqref{eq:collecting_terms}, and simplifying completes the proof. \textcolor{red}{define $\Delta_E$, help simplifying}

\section{Proofs of Helper Lemmas for Theorem  \ref{thm:potential_outcome_convergence_rate}.}
\label{sec:helper_lemma_proofs}
In this section we provide proofs of Lemmas \ref{lem:w_tilde_transfer_outcomes}, \ref{lem:l1_bound_w_tilde} and Proposition \ref{prop:pcr_convergence_rate} which were required for the Proof of Theorem \ref{thm:potential_outcome_convergence_rate}.  

\subsection{Proof of Lemma \ref{lem:w_tilde_transfer_outcomes}}
\label{subsec:proof_of_w_tilde_transfer_outcomes}

By Assumption \ref{ass:observation_model} and \ref{ass:donor_set_identification} (b), we have
\begin{align*}
    \E[Y_n^{(\pi)}] & = \E[\langle \balpha_n, \bchi^{\pi} \rangle + \epsilon_n^{\pi}] \\
    & =  \E[\langle \balpha_n, \bchi^{\pi} \rangle ] \\
    & =  \sum_{u \in \mathcal{I}}w^n_u\E[\langle \balpha_u, \bchi^{\pi} \rangle] \\
    & = \sum_{u \in \mathcal{I}}w^n_u \E[Y_u^{(\pi)}] \\
    & = \E[\bY_{\mathcal{I}}^{(\pi)}]^T \bw^{n}
\end{align*}
From Assumption \ref{ass:rowspace_inclusion}, we have that  $\E[\bY_{\mathcal{I}}^{(\pi)}] = \mathcal{P}_{V_{\mathcal{I}}^{(\Pi_n)}} \E[\bY_{\mathcal{I}}^{(\pi)}]$. Substituting this into the equation above completes the proof. 


\subsection{Proof of Lemma \ref{lem:l1_bound_w_tilde}}
\label{subsec:proof_of_l1_bound_w_tilde}
For simplicity, denote $\E[\bY_n^{(\Pi_n)}] = \E[\bY^{(\Pi_n)}]$.  By definition, $\tilde{\bw}^n$ is the solution to the following optimization program 
\begin{align}
\min_{ \bw \in \mathbb{R}^{|\mathcal{I}|}} \quad & ||{\bw}||_2 \nonumber \\
\textrm{s.t.} \quad & \E[\bY^{(\Pi_n)}] = \E[\bY_{\mathcal{I}}^{(\Pi_n)}]\bw
\label{eq:linear_system_donor_set}
\end{align}

\noindent Let $\bU_{\mathcal{I}}^{(\Pi_n)}, \mathbf{\Sigma}_{\mathcal{I}}^{(\Pi_n)}, \bV_{\mathcal{I}}^{(\Pi_n)}$ denote the SVD of $\E[\bY_{\mathcal{I}}^{(\Pi_n)}]$. Further, let $\bU_{\mathcal{I}}^{(\Pi_n),r_n}, \mathbf{\Sigma}_{\mathcal{I}}^{(\Pi_n),r_n}, \bV_{\mathcal{I}}^{(\Pi_n),r_n}$ denote the rank $r_n$ truncation of the SVD. Then, define $\bw_{r_n} =  \bV_{\mathcal{I}}^{(\Pi_n),r_n} (\mathbf{\Sigma}_{\mathcal{I}}^{(\Pi_n),r_n})^{\dagger} (\bU_{\mathcal{I}}^{(\Pi_n),r_n})^T \E[\bY^{(\Pi_n)}]$, where $\dagger$ is pseudo-inverse. We first show that $\bw_{r_n}$ is a solution to \eqref{eq:linear_system_donor_set}. 


\begin{align*}
    \E[\bY_{\mathcal{I}}^{(\Pi_n)}] \bw_{r_n} &= \left( \bU_{\mathcal{I}}^{(\Pi_n)} \mathbf{\Sigma}_{\mathcal{I}}^{(\Pi_n)} (\bV_{\mathcal{I}}^{(\Pi_n)})^T \right) \bV_{\mathcal{I}}^{(\Pi_n),r_n} (\mathbf{\Sigma}_{\mathcal{I}}^{(\Pi_n),r_n})^{\dagger} (\bU_{\mathcal{I}}^{(\Pi_n),r_n})^T \E[\bY^{(\Pi_n)}] \\
    & = \left(\sum^{r_n}_{i=1} s_i u_i v^{T}_i\right) \left(\sum^{r_n}_{j=1} \frac{1}{s_j}v_j u^T_j \E[\bY^{(\Pi_n)}]\right) \\
    & = \sum^{r_n}_{i,j=1} \frac{s_i}{s_j} u_i v^T_i v_j u_j^T \E[\bY^{(\Pi_n)}] \\
    & = \sum^{r_n}_{i=1} u_i u^T_i \E[\bY^{(\Pi_n)}] \\
    & = \E[\bY^{(\Pi_n)}] 
\end{align*}


Next, we bound $\lVert \bw_{r_n} \rVert_2$ using Assumptions \ref{ass:boundedness_potential_outcome} and \ref{ass:balanced_spectrum} as follows 
\begin{align*}
    \lVert \bw_{r_n} \rVert_2 & \leq \lVert (\mathbf{\Sigma}_{\mathcal{I}}^{(\Pi_n),r_n})^{\dagger} \rVert_2  \lVert \E[\bY^{(\Pi_n)}] \rVert_2 \\
    & \leq \frac{\sqrt{|\Pi_n|}}{s_{r_n}(\E[\bY_{\mathcal{I}}^{(\Pi_n)}])} \\
    & \leq \sqrt{\frac{cr_n}{|\mathcal{I}|}}
\end{align*}
Therefore, we have 
\begin{align*}
    \lVert \Tilde{\bw}^n \rVert_1 \leq \sqrt{|\mathcal{I}|} \lVert \Tilde{\bw}_{r_n} \rVert_2 \leq \sqrt{cr_n}
\end{align*}



% \subsection{Proof of Lemma \ref{lem:projection_delta_w_bound}}
% \label{subsubsec:proof_lemma_projection_delta_w_bound}

% \noindent First, we introduce some necessary notation required for the proof. Let $\hat{\E}\left[\bY_{\mathcal{I}}^{(\Pi_n)} \right] = \hat{\bU}_{\mathcal{I}}^{(\Pi_n)}\hat{\bS}_{\mathcal{I}}^{(\Pi_n)}\hat{\bV}_{\mathcal{I}}^{(\Pi_n)}$ denote the rank $r_n$ SVD of $\hat{\E}\left[\bY_{\mathcal{I}}^{(\Pi_n)} \right]$. Then, to establish Lemma \ref{lem:projection_delta_w_bound}, consider the following decomposition:
% \begin{equation*}
%     \mathcal{P}_{V_{\mathcal{I}}^{(\Pi_n)}}\Delta^n_w = \left(\mathcal{P}_{V_{\mathcal{I}}^{(\Pi_n)}} - \mathcal{P}_{\hat{V}_{\mathcal{I}}^{(\Pi_n)}}  \right)\Delta^n_w  + \mathcal{P}_{\hat{V}_{\mathcal{I}}^{(\Pi_n)}}\Delta^n_w 
% \end{equation*}
% \noindent We bound each of these terms separately again. \\

% \noindent \emph{Bounding Term 1}. We have
% \begin{equation}
% \label{eq:projection_operator_error_cauchy}
%      \lVert \left(\mathcal{P}_{V_{\mathcal{I}}^{(\Pi_n)}} - \mathcal{P}_{\hat{V}_{\mathcal{I}}^{(\Pi_n)}}  \right)\Delta^n_w \rVert_2  \leq \left\lVert \mathcal{P}_{V_{\mathcal{I}}^{(\Pi_n)}} - \mathcal{P}_{\hat{V}_{\mathcal{I}}^{(\Pi_n)}}  \right\rVert_{\text{op}} \lVert \Delta^n_w \rVert_2
% \end{equation}

% \begin{theorem} [Wedin's Theorem \cite{wedin1972perturbation}]
% \label{thm:wedin_theorem}
% Given $\mathbf{A},\mathbf{B} \in \R^{m \times n}$, let $(\bU,\bV),(\hat{\bU},\hat{\bV})$ denote their respective left and right singular vectors. Further, let $(\bU_k,\bV_k) \in $(respectively, $(\hat{\bU}_k,\hat{\bV}_k)$) correspond to the truncation of $(\bU,\bV)$ (respectively, $(\hat{\bU},\hat{\bV})$), respectively, that retains the columns correspondng to the top $k$ singular values of $\mathbf{A}$ (respectively, $\mathbf{B}$). Let $s_i$ represent the $i$-th singular values of $A$. Then, $\max(\lVert \mathcal{P}_{U_k} - \mathcal{P}_{\hat{U}_k}\rVert_{\text{op}}, \lVert \mathcal{P}_{V_k} - \mathcal{P}_{\hat{V}_k}\rVert_{\text{op}}) \leq \frac{2\lVert \mathbf{A} - \mathbf{B} \rVert_{\text{op}}}{s_{k}-s_{k+1}}$   
% \end{theorem}

% \noindent Applying Theorem \ref{thm:wedin_theorem} gives us 
% \begin{align}
% \max\left(\left\lVert \mathcal{P}_{U_{\mathcal{I}}^{(\Pi_n)}} - \mathcal{P}_{\hat{U}_{\mathcal{I}}^{(\Pi_n)}}  \right\rVert_{\text{op}}, \left\lVert \mathcal{P}_{V_{\mathcal{I}}^{(\Pi_n)}} - \mathcal{P}_{\hat{V}_{\mathcal{I}}^{(\Pi_n)}}  \right\rVert_{\text{op}} \right) & \leq  \frac{2\lVert \E[\bY_{\mathcal{I}}^{(\Pi_n)}] - \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n)}] \rVert_{\text{op}}}{s_{r_n} - s_{r_n + 1}}  \nonumber \\
% & \leq \frac{2\sqrt{|\mathcal{I}||\Pi_n|}\lVert \E[\bY_{\mathcal{I}}^{(\Pi_n)}] - \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n)}] \rVert_{\text{max}}}{s_{r_n} - s_{r_n + 1}} \nonumber  \\
% & = \frac{2\sqrt{|\mathcal{I}||\Pi_n|}\Delta_E}{s_{r_n} - s_{r_n + 1}} \nonumber \\ 
% & = \frac{2\sqrt{|\mathcal{I}||\Pi_n|}\Delta_E}{s_{r_n}} \label{eq:projection_operator_error_operator_bound}
% \end{align}
% \noindent where the last equality follows from the fact that  $\text{rank}(\E[\bY_{\mathcal{I}}^{\Pi_n}]) = r_n$, hence $s_{r_n + 1} = 0$. Now, plugging Assumption \ref{ass:balanced_spectrum}, \eqref{eq:projection_operator_error_operator_bound}  into \eqref{eq:projection_operator_error_cauchy} gives us
% \begin{equation}
% \label{eq:projection_operator_error_bound_simplified}
%     \max\left(\left\lVert \mathcal{P}_{V_{\mathcal{I}}^{(\Pi_n)}} - \mathcal{P}_{\hat{V}_{\mathcal{I}}^{(\Pi_n)}}  \right\rVert_{\text{op}}, \left\lVert \mathcal{P}_{V_{\mathcal{I}}^{(\Pi_n)}} - \mathcal{P}_{\hat{V}_{\mathcal{I}}^{(\Pi_n)}}  \right\rVert_{\text{op}} \right) \leq C\sqrt{r_n}\Delta_E 
% \end{equation}
% Substituting the result of Proposition \ref{prop:pcr_convergence_rate} and \eqref{eq:projection_operator_error_bound_simplified} into \eqref{eq:projection_operator_error_cauchy} gives us
% \begin{equation}
% \label{eq:projection_operator_term1_bound}
%       \left \lVert \left(\mathcal{P}_{V_{\mathcal{I}}^{(\Pi_n)}} - \mathcal{P}_{\hat{V}_{\mathcal{I}}^{(\Pi_n)}}  \right)\Delta^n_w \right \rVert_2 = O_p \left(\log^3\left(|\Pi_n||\mathcal{I}|\right) r_n^{3/2} \lVert \Tilde{\bw}^{n} \rVert_2 \left[\frac{ \Delta_E  }{\min\{\sqrt{|\Pi_n|},\sqrt{|\mathcal{I}|\}}}  + \Delta^2_E \right] \right)
% \end{equation} \\

% \noindent To further simplify \eqref{eq:projection_operator_term1_bound}, we substitute the result of Lemma \ref{lem:l1_bound_w_tilde}

% \noindent Substituting the Lemma \ref{lem:l1_bound_w_tilde} into \eqref{eq:projection_operator_term1_bound} gives us
% \begin{equation}
% \label{eq:projection_operator_term1_bound_simplified}
%       \left \lVert \left(\mathcal{P}_{V_{\mathcal{I}}^{(\Pi_n)}} - \mathcal{P}_{\hat{V}_{\mathcal{I}}^{(\Pi_n)}}  \right)\Delta^n_w \right \rVert_2 = {O_p} \left( \log^3\left(|\Pi_n||\mathcal{I}|\right) r_n^{2}\left[\frac{\Delta_E  }{\sqrt{|\mathcal{I}|}\min\{\sqrt{|\Pi_n|},\sqrt{|\mathcal{I}|\}}}  + \frac{\Delta^2_E}{\sqrt{|\mathcal{I}|}} \right] \right)
% \end{equation}





% \noindent  \emph{Bounding Term 2.}  We introduce some necessary notation required to bound the second term. 
% Let $\hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}] = \sum^{r_n}_{l=1}\hat{s}_l\hat{\mu}_l\hat{v}'_l$ denote the $r_n$ decomposition of $\hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n)}]$. Let, $\hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}] = \hat{\bU}_{\mathcal{I}}^{(\Pi_n)}\hat{\bS}_{\mathcal{I}}^{(\Pi_n)}(\hat{\bV}_{\mathcal{I}}^{(\Pi_n)})^T$. 
% %
% Further, define $\bepsilon^{\Pi_n} = [\epsilon_n^{\pi}: \pi \in \Pi_n] \in \R^{|\Pi_n|}$. \\
% %
% \noindent Then to begin, note that since $\hat{\bV}^{(\Pi_n)}_{\mathcal{I}}$ is a isometry, we have that
% \begin{equation*}
%     \lVert \mathcal{P}_{\hat{V}_{\mathcal{I}}^{(\Pi_n)}}\Delta^n_w  \rVert^2_2  = \lVert (\hat{\bV}^{(\Pi_n)}_{\mathcal{I}})^T\Delta^n_w \rVert^2_2
% \end{equation*}

% \noindent To upper bound $\lVert (\hat{\bV}^{(\Pi_n)}_{\mathcal{I}})^T \Delta^n_w \rVert^2_2$ as follows, consider 
% \begin{equation*}
%    \lVert \hat{\E}[\bY^{(\Pi_n)}_{\mathcal{I}}] \Delta^n_w\rVert^2_2 = \left( (\hat{\bV}^{(\Pi_n)}_{\mathcal{I}})^T\Delta^n_w \right)^T \left(\hat{\bS}_{\mathcal{I}}^{(\Pi_n)}\right)^2 \left( (\hat{\bV}^{(\Pi_n)}_{\mathcal{I}})^T \Delta^n_w \right) \geq \hat{s}^2_{r_n} \lVert (\hat{\bV}^{(\Pi_n)}_{\mathcal{I}})^T \Delta^n_w  \rVert^2_2
% \end{equation*}

% \noindent Using the two equations above gives us
% \begin{equation}
% \label{eq:projection_term2_intermediate_bound1}
%     \lVert \mathcal{P}_{\hat{V}_{\mathcal{I}}^{(\Pi_n)}}\Delta^n_w  \rVert^2_2   \leq \frac{ \lVert \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] \Delta^n_w\rVert^2_2}{\hat{s}^2_{r_n}}
% \end{equation}

% \noindent To bound the numerator in \eqref{eq:projection_term2_intermediate_bound1}, note that  by definition $\E[\bY^{(\Pi_n)}] = \E[\bY_{\mathcal{I}}^{(\Pi_n)}] \Tilde{\bw}^n$. Using this observation, we have
% \begin{align}
%     \lVert \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] \Delta^n_w\rVert^2_2 & \leq 2 \lVert \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] \hat{\bw}^n - \E[\bY^{(\Pi_n)}] \rVert^2_2 + 2\lVert \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] \tilde{\bw}^n - \E[\bY^{(\Pi_n)}] \rVert^2_2 \nonumber \\
%     & = 2\lVert \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] \hat{\bw}^n - \E[\bY^{(\Pi_n)}] \rVert^2_2 + 2\lVert (\hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] - \E[\bY_{\mathcal{I}}^{(\Pi_n)}])\tilde{\bw}^n  \rVert^2_2\label{eq:term2_numerator_bound}
% \end{align} 
% \noindent To proceed, we then use the following inequality: for any $\mathbf{A} \in \mathbb{R}^{a \times b}, v \in \mathbb{R}^b$, we have
% \begin{equation}
% \label{eq:l2_infty_inequality}
%     \lVert \mathbf{A}v \rVert_2 = \lVert \sum^b_{j =1} \mathbf{A}_{.j} v_j \rVert_2 \leq \left( \max_{j \leq b} \lVert \mathbf{A}_{.j} \rVert_2 \right) \left( \sum^b_{j=1} v_j \right) = \lVert \mathbf{A} \rVert_{2,\infty} \lVert v \rVert_1
% \end{equation} 
% \noindent Substituting \eqref{eq:term2_numerator_bound} into \eqref{eq:projection_term2_intermediate_bound1} and then applying inequality \eqref{eq:l2_infty_inequality} gives us  
% \begin{equation}
% \label{eq:projection_term2_intermediate_bound2}
%      \lVert \mathcal{P}_{\hat{V}_{\mathcal{I}}^{(\Pi_n)}}\Delta^n_w  \rVert^2_2  \leq \frac{2}{\hat{s}^2_{r_n}}\left(\lVert \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] \hat{\bw}^n - \E[\bY^{(\Pi_n)}] \rVert^2_2  + \lVert \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] - \E[\bY_{\mathcal{I}}^{(\Pi_n)}] \rVert^2_{2,\infty} \lVert \tilde{\bw}^n \rVert^2_1\right)
% \end{equation}
% Next, we bound $\lVert \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] \hat{\bw}^n - \E[\bY^{(\Pi_n)}] \rVert^2_2$. To this end, note that Assumption \ref{ass:observation_model} implies that
% \begin{align}
%      &\lVert \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] \hat{\bw}^n - \bY^{(\Pi_n)} \rVert^2_2 \nonumber \\
%      & = \lVert \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] \hat{\bw}^n - \E[\bY^{(\Pi_n)}] - \bepsilon^{\Pi_n} \rVert^2_2 \nonumber \\
%     & =  \lVert \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] \hat{\bw}^n - \E[\bY^{(\Pi_n)}] \rVert^2_2 + \lVert \bepsilon^{\Pi_n} \rVert^2_2 - 2\langle  \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] \hat{\bw}^n - \E[\bY^{(\Pi_n)}], \bepsilon^{\Pi_n} \rangle \label{eq:pcr_training_error_bound_noiseless}
% \end{align}
% \noindent Next, we proceed by calling upon Property 4.1 of \cite{agarwal2020principal} which states that $\hat{\bw}^n$ as given by \eqref{eq:pcr_linear_model_def} is the unique solution to the following convex program: 
% \begin{align}
% \label{eq:hat_w_min_l2_property}
% & \min_{\bw \in \mathbb{R}^{|\mathcal{I}|}} \quad  ||{\bw}||_2 \nonumber \\
% & \textrm{s.t. } \bw \in \argmin_{\bw \in \mathbb{R}^{|\mathcal{I}|}} \lVert \bY^{(\Pi_n)} - \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}]\bw \rVert^2_2
% \end{align}
% Using this property, we have that
% \begin{align}
%     & \lVert \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] \hat{\bw}^n - \bY^{(\Pi_n)} \rVert^2_2 \nonumber 
%     \\ & \leq   \lVert \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] \tilde{\bw}^n - \bY^{(\Pi_n)} \rVert^2_2 \nonumber \\
%     & = \lVert \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] \tilde{\bw}^n - \E[\bY^{(\Pi_n)}] - \bepsilon^{\Pi_n}  \rVert^2_2 \nonumber\\
%     & = \lVert \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] \tilde{\bw}^n - \E[\bY_{\mathcal{I}}^{(\Pi_n)}]\tilde{\bw}^n  - \bepsilon^{\Pi_n}  \rVert^2_2 \nonumber \\
%     & = \lVert (\hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] - \E[\bY_{\mathcal{I}}^{(\Pi_n)}])\tilde{\bw}^n \rVert^2_2 + \lVert \bepsilon^{\Pi_n} \rVert^2_2 - 2 \langle (\hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] - \E[\bY_{\mathcal{I}}^{(\Pi_n)}])\tilde{\bw}^n, \bepsilon^{\Pi_n} \rangle \label{eq:pcr_training_error_bound}
% \end{align}

% \noindent Substituting \eqref{eq:pcr_training_error_bound_noiseless} and \eqref{eq:pcr_training_error_bound} into \eqref{eq:projection_term2_intermediate_bound2} and using \eqref{eq:l2_infty_inequality}, we get
% \begin{align*}
% & \lVert \hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}] \hat{\bw}^n - \E[\bY^{(\Pi_n)}] \rVert^2_2 \\
% & \leq \lVert (\hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),r_n}] - \E[\bY_{\mathcal{I}}^{(\Pi_n)}])\tilde{\bw}^n \rVert^2_2 + 2 \langle (\hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}])\Delta_w^n, \bepsilon^{\Pi_n} \rangle \\
% & \leq \lVert (\hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),r_n}] - \E[\bY_{\mathcal{I}}^{(\Pi_n)}])\rVert^2_{2,\infty} \lVert \tilde{\bw}^n  \rVert^2_1 + 2 \langle (\hat{\E}[\bY^{(\Pi_n),r_n}_{\mathcal{I}}])\Delta_w^n, \bepsilon^{\Pi_n} \rangle 
% \end{align*}
    
% \noindent Then substituting this equation into \eqref{eq:projection_term2_intermediate_bound2} gives us 
% \begin{equation}
% \label{eq:projection_operator_term2_intermediate_bound}
%    \lVert \mathcal{P}_{\hat{V}_{\mathcal{I}}^{(\Pi_n)}}\Delta^n_w \rVert^2_2 \leq \frac{4}{\hat{s}^2_{r_n}}\left(\lVert \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}] - \E[\bY_{\mathcal{I}}^{(\Pi_n)}] \rVert^2_{2,\infty} \lVert \Tilde{\bw}^n \rVert^2_1 +  \langle  \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}] \Delta^n_w, \bepsilon^{\Pi_n} \rangle \right)
% \end{equation}
% We state three lemmas that help us bound the equation above with their proofs given in Appendices \ref{subsubsec:proof_singular_value_lower_bound}, \ref{subsubsec:proof_of_lemma_rank_r_approximation_l2_infty_bound} and \ref{subsubsec:proof_of_lemma_rank_r_approximaton_noise_inner_product_bound} respectively. 
% \begin{lemma}
% \label{lem:singular_value_lower_bound}
% Let the set-up of Theorem \ref{thm:potential_outcome_convergence_rate} hold. Then, 
% \begin{equation*}
%     \hat{s}_{r_n} - s_{r_n} = O_p(1)
% \end{equation*}
% \end{lemma}

% \begin{lemma}
% \label{lem:rank_r_approximation_l2_infty_bound}
% Let the set-up of Theorem \ref{thm:potential_outcome_convergence_rate} hold. Then for a universal constant $C > 0$, we have 
% \begin{equation}
%    \lVert \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}] - \E[\bY_{\mathcal{I}}^{(\Pi_n)}] \rVert_{2,\infty} \leq C \sqrt{r_n|\Pi_n|} \Delta_E
% \end{equation}
% \end{lemma}

% \begin{lemma} Let the set-up of Theorem \ref{thm:potential_outcome_convergence_rate} hold. Then, 
% \label{lem:rank_r_approximaton_noise_inner_product_bound}
%  \begin{equation}
%   \langle  \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}] \Delta^n_w, \bepsilon^{\Pi_n} \rangle = O_p \left(\sqrt{|\Pi_n|} + r_n +  \lVert \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}] - \E[\bY_{\mathcal{I}}^{(\Pi_n)}] \rVert_{2,\infty} \lVert \Tilde{\bw}^n \rVert_1 \right)
% \end{equation}
% \end{lemma}
% \noindent Using the results of three lemmas above, applying Assumption \ref{ass:balanced_spectrum} in \eqref{eq:projection_operator_term2_intermediate_bound}, and then simplifying gives us 
% \begin{equation}
% \label{eq:projection_operator_term2_bound}
%     \lVert \mathcal{P}_{\hat{V}_{\mathcal{I}}^{(\Pi_n)}}\Delta^n_w \rVert_2  = O_p \left(\frac{r_n\Delta_E\lVert \Tilde{\bw}^n \rVert_1}{\sqrt{|\mathcal{I}|}} + \frac{r_n\left( 1 + \sqrt{\Delta_E\lVert \Tilde{\bw}^n \rVert_1}\right)}{\sqrt{|\mathcal{I}|}|\Pi_n|^{1/4}}\right)
% \end{equation}
% \noindent This concludes the proof for term 2. Using the result of Lemma \ref{lem:l1_bound_w_tilde}, we have that $\lVert \Tilde{\bw}^n \rVert_1 \leq c\sqrt{r_n}$. Substituting this into \eqref{eq:projection_operator_term2_bound} gives us
% \begin{equation}
% \label{eq:projection_operator_term2_bound_simplified}
%     \lVert \mathcal{P}_{\hat{V}_{\mathcal{I}}^{(\Pi_n)}}\Delta^n_w \rVert_2  = O_p \left(\frac{r_n^{3/2}\Delta_E}{\sqrt{|\mathcal{I}|}} + \frac{r_n\left( 1 + \sqrt{\Delta_E}r^{1/4}_n\right)}{\sqrt{|\mathcal{I}|}|\Pi_n|^{1/4}}\right)
% \end{equation}

% \noindent \emph{Collecting Terms. }Combining the results of \eqref{eq:projection_operator_term1_bound_simplified} and \eqref{eq:projection_operator_term2_bound_simplified}, gives us
% \begin{align*}
% & \lVert \mathcal{P}_{V_{\mathcal{I}}^{(\Pi_n)}}\Delta^n_w \rVert_2 \nonumber \\
% & = O_p \left( \log^{3}(|\Pi_n||\mathcal{I}|)r_n^{2}\left[\frac{\Delta_E  }{\sqrt{|\mathcal{I}|}\min\{\sqrt{|\Pi_n|},\sqrt{|\mathcal{I}|\}}}  + \frac{\Delta^2_E}{\sqrt{|\mathcal{I}|}} \right]  + \frac{r_n^{3/2}\Delta_E}{\sqrt{|\mathcal{I}|}} + \frac{r_n\left( 1 + \sqrt{\Delta_E}r^{1/4}_n\right)}{\sqrt{|\mathcal{I}|}|\Pi_n|^{1/4}}  \right) 
% \end{align*}

% \subsubsection{Proof of Lemma \ref{lem:singular_value_lower_bound}}
% \label{subsubsec:proof_singular_value_lower_bound}
% We first state Weyl's inequality which will be useful for us to establish the results. 
% \begin{theorem}[Weyl's Inequality]
% \label{thm:weyl_inequality}
% Given two matrices $\mathbf{A},\mathbf{B} \in \R^{m \times n}$, let $s_i$ and $\hat{s}_i$ denote the $i$-th singular values of $\mathbf{A}$ and $\mathbf{B}$ respectively. Then, for all, $i \leq \min\{n,m\}$, we have $\left| s_i - \hat{s}_i \right| \leq \left\lVert\mathbf{A} - \mathbf{B} \right\rVert_{\text{op}}$
% \end{theorem}
% \noindent Using Weyl's inequality gives us 
% \begin{align*}
%     | \hat{s}_{r_n} - s_{r_n} | & \leq \lVert \E[\bY_{\mathcal{I}}^{(\Pi_n)}] - \hat{E}[\bY_{\mathcal{I}}^{(\Pi_n)}] \rVert_{\text{op}} \\
%     & \leq \sqrt{|\mathcal{I}||\Pi_n|}\Delta_E
% \end{align*}
% \noindent Using the inequality above and Assumption \ref{ass:balanced_spectrum}, we have 
% \begin{align*}
% \hat{s}_{r_n} & \geq s_{r_n} - \sqrt{|\mathcal{I}|\Pi_n}\Delta_E \\
%         & = s_{r_n}\left(1 - \frac{\sqrt{|\mathcal{I}|\Pi_n}\Delta_E}{s_{r_n}}\right) \\
%         & \geq s_{r_n}\left(1 - \sqrt{r_n}\Delta_E \right) \\
% \end{align*}
% Then, substituting \eqref{eq:delta_E_subsitution} into the equation above gives us that
% \begin{equation*}
%     \frac{\hat{s}_{r_n}}{s_{r_n}} \geq \left(1 - C\sqrt{\frac{r_ns^2p}{M}}\right)
% \end{equation*}
% holds with high probability for some universal constant $C \geq 0$. Finally, using the assumption that $M = \omega(r_n^2s^2p)$ yields the claimed result. 
    

% \subsubsection{Proof of Lemma \ref{lem:rank_r_approximation_l2_infty_bound}}
% \label{subsubsec:proof_of_lemma_rank_r_approximation_l2_infty_bound}
% For notational simplicity, let $\hat{\bU}_{r_n},\hat{\bS}_{r_n},\hat{\bV}_{r_n}$ denote $\hat{\bU}_{\mathcal{I}}^{(\Pi_n)},\hat{\bS}_{\mathcal{I}}^{(\Pi_n)},\hat{\bV}_{\mathcal{I}}^{(\Pi_n)}$ respectively.  For a matrix $\mathbf{A}$, let $A_{.,j}$ denote its $j$-th column. Additionally, denote  $\Delta_{j} = \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}]_{.,j} - \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j}$. Then,
% \begin{align*}
%     & \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}]_{.,j} - \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} \\
%     & = \left(\hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}]_{.,j} - \hat{\bU}_{r_n}\hat{\bU}^T_{r_n} \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} \right) + \left(\hat{\bU}_{r_n}\hat{\bU}^T_{r_n} \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j}  - \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} \right)
% \end{align*}
% \noindent We have that $\left(\hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}]_{.,j} - \hat{\bU}_{r_n}\hat{\bU}^T_{r_n} \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} \right)$ belongs to the subspace spanned by the column vectors of $\hat{\bU}_{r_n}$, while $\left(\hat{\bU}_{r_n}\hat{\bU}^T_{r_n} \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j}  - \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} \right)$ belongs to its orthogonal complement. Therefore, 
% \begin{align*}
%      & \lVert \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}]_{.,j} - \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} \rVert^2_2 \\
%       & = \left\lVert\hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}]_{.,j} - \hat{\bU}_{r_n}\hat{\bU}^T_{r_n} \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} \right\rVert^2_2 + \left\lVert\hat{\bU}_{r_n}\hat{\bU}^T_{r_n} \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j}  - \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} \right\rVert^2_2
% \end{align*}

% \noindent \emph{Bounding $\left\lVert\hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}]_{.,j} - \hat{\bU}_{r_n}\hat{\bU}^T_{r_n} \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} \right\rVert^2_2$}. 
% Observe that, we have 
% \begin{align*}
%     \hat{\bU}_{r_n}\hat{\bU}^T_{r_n}\hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} & =   \hat{\bU}_{r_n}\hat{\bU}^T_{r_n} \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n)}]\mathbf{e_{j}}  = \hat{\bU}_{r_n}\hat{\bU}^T_{r_n}\hat{\bU}_{\mathcal{I}}^{(\Pi_n)}\hat{\bS}_{\mathcal{I}}^{(\Pi_n)}\hat{\bV}_{\mathcal{I}}^{(\Pi_n)} \mathbf{e_{j}} \\
%     & =  \hat{\bU}_{r_n}\hat{\bS}_{r_n}\hat{\bV}^T_{r_n}\mathbf{e}_j =    \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}]_{.,j}
% \end{align*}
% \noindent Therefore, we have
% \begin{align*}
%     \left\lVert\hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}]_{.,j} - \hat{\bU}_{r_n}\hat{\bU}^T_{r_n} \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} \right\rVert^2_2  & = \left\lVert\hat{\bU}_{r_n}\hat{\bU}^T_{r_n}\hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} - \hat{\bU}_{r_n}\hat{\bU}^T_{r_n} \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} \right\rVert^2_2 \\
%     & \leq \left\lVert\hat{\bU}_{r_n}\hat{\bU}^T_{r_n} \right\rVert^2_2 \left \lVert \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} - \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j}\right\rVert^2_2 \\ 
%     & \leq |\Pi_n|\Delta^2_E
% \end{align*} 

% \noindent \emph{Bounding $\left\lVert\hat{\bU}_{r_n}\hat{\bU}^T_{r_n} \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j}  - \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} \right\rVert^2_2$.} Note that $ \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} = \bU_{\mathcal{I}}^{(\Pi_n)}\left(\bU_{\mathcal{I}}^{(\Pi_n)}\right)^T\E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j}$. Using Assumption \ref{ass:boundedness_potential_outcome} and \eqref{eq:projection_operator_error_bound_simplified}, we have 
% \begin{align*}
%     \left\lVert\hat{\bU}_{r_n}\hat{\bU}^T_{r_n} \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j}  - \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} \right\rVert^2_2 & \leq \left\lVert \hat{\bU}_{r_n}\hat{\bU}^T_{r_n} -  \bU_{\mathcal{I}}^{(\Pi_n)}\left(\bU_{\mathcal{I}}^{(\Pi_n)}\right)^T \right\rVert^2_2 \lVert \E[\bY_{\mathcal{I}}^{(\Pi_n)}]_{.,j} \rVert^2_2 \\
%     & \leq \left\lVert \hat{\bU}_{r_n}\hat{\bU}^T_{r_n} -  \bU_{\mathcal{I}}^{(\Pi_n)}\left(\bU_{\mathcal{I}}^{(\Pi_n)}\right)^T \right\rVert^2_2 \left|\Pi_n \right| \\
%     & \leq C r_n |\Pi_n| \Delta^2_E
% \end{align*}
% \noindent for a universal constant $C > 0$. 
% \noindent Combining the two bounds gives us, 
% \begin{equation*}
%     \max_{j} \ \Delta_j \leq C\sqrt{r_n|\Pi_n|}\Delta_E
% \end{equation*}
% \noindent for a universal constant $C > 0.$

% \subsubsection{Proof of Lemma \ref{lem:rank_r_approximaton_noise_inner_product_bound}}
% \label{subsubsec:proof_of_lemma_rank_r_approximaton_noise_inner_product_bound}

    
% The proof of Lemma \ref{lem:rank_r_approximaton_noise_inner_product_bound} follows from adapting the notation of Lemma H.5 in \cite{agarwal2020synthetic} to that used in this paper. Specifically, we have the notational changes established in Table \ref{tab:notational_changes}, as well as the following changes: $r_{pre} = r_n, \bY_{pre,\mathcal{I}^{(d)}}^{r_{pre}} = \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}], \E[\bY_{pre,\mathcal{I}^{(d)}}], \epsilon_{pre,n} = \bepsilon^{\Pi_n}, T_0 = \Pi_n$  where the left hand side of each equality is the notation used in \cite{agarwal2020synthetic} , and the right hand side is the notation used in this work. Using the notation established, we can use the result of Lemma H.5 in \cite{agarwal2020synthetic} to give us 
% \begin{equation*}
%       \langle  \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}] \Delta^n_w, \bepsilon^{\Pi_n} \rangle = O_p \left(\sqrt{|\Pi_n|} + r_n +  \lVert \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n),{r_n}}] - \E[\bY_{\mathcal{I}}^{(\Pi_n)}] \rVert_{2,\infty} \lVert \Tilde{\bw}^n \rVert_1 \right)
% \end{equation*}
% which completes the proof. 



\subsection{Proof of Proposition \ref{prop:pcr_convergence_rate}}
\label{subsec:pcr_proofs}
We prove Proposition \ref{prop:pcr_convergence_rate}, which also serves as the finite-sample analysis of the vertical regression procedure (step 2 of \method) done via principal component regression. The proof follows from adapting the notation of Proposition E.3 in \cite{agarwal2021causal} to that used in this paper. Specifically, we present Table \ref{tab:notational_changes} below that matches their notation to ours. 
This gives the result,
\begin{equation*}
    \lVert \hat{\bw}^n - \Tilde{\bw}^n \rVert_2 = O_p \left(\log^{3}(|\Pi_n||\mathcal{I}|)r_n\lVert \Tilde{\bw}^{n} \rVert_2\left[\frac{ 1 }{\min\{\sqrt{|\Pi_n|},\sqrt{|\mathcal{I}|\}}}  + \Delta_E \right] \right)
\end{equation*}
\begin{table}[H]
\centering
\begin{tabular}{||c c||} 
 \hline
 Notation of \cite{agarwal2021causal} & Our Notation \\ [1ex] 
 \hline
 $\bY$ & $\bY_{\Pi_n}$  \\ [1ex]
 \hline
 $\bX$ & $\E[\bY_{\mathcal{I}}^{(\Pi_n)}]$ \\  [1ex]
 \hline
 $\bZ$ &  $\hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n)}]$  \\ [1ex]
 \hline 
 $n$ & $|\Pi_n|$ \\
 \hline 
 $p$ & $|\mathcal{I}|$ \\
 \hline 
$\bbeta^*$ & $\Tilde{\bw}$ \\
\hline
$\hat{\bbeta}$ & $\hat{\bw}$ \\
\hline
$\Delta_E$ & $\Delta_E$ \\
\hline 
$r$ & $r_n$ \\
\hline 
$\phi^{lr}$ & $0$ \\ [1ex]
 \hline
 $\Bar{A}$ & $1$ \\ 
 \hline
 $\Bar{K}$ & 0  \\ [1ex] 
 \hline
 $K_{a}, \kappa, \Bar{\sigma}$ & $C\sigma$ \\
 \hline 
 $\rho_{min}$ & 1 \\
 \hline 
 \end{tabular}
 \vspace{1mm}
\caption{A summary of the main notational differences between our setting and that of \cite{agarwal2021causal}.}
\label{tab:notational_changes}
\end{table}


%\begin{center}

%\end{center}





%\begin{lemma} 
%\label{lem:projection_delta_w_bound}
%Let the set-up of Theorem \ref{thm:potential_outcome_convergence_rate} hold. Then, 
%\begin{align}
%& \lVert \mathcal{P}_{V_{\mathcal{I}}^{(\Pi_n)}}\Delta^n_w \rVert_2 \nonumber \\
%& = O_p\left(\log^{3}\left(|\Pi_n||\mathcal{I}|\right)  r_n^{2}\left[\frac{\Delta_E  }{\sqrt{|\mathcal{I}|}\min\{\sqrt{|\Pi_n|},\sqrt{|\mathcal{I}|\}}}  + \frac{\Delta^2_E}{\sqrt{|\mathcal{I}|}} \right] + \frac{r_n^{3/2}\Delta_E}{\sqrt{|\mathcal{I}|}} + \frac{r_n\left( 1 + \sqrt{\Delta_E}r^{1/4}_n\right)}{\sqrt{|\mathcal{I}|}|\Pi_n|^{1/4}}  \right) \label{eq:projection_delta_w_bound}
%\end{align}
%\begin{equation}
%\label{eq:projection_delta_w_bound}
%    \lVert \mathcal{P}_{\hat{V}_{\mathcal{I}}^{(\Pi_n)}}\Delta^n_w \rVert_2  = O_p \left(\left(\log^3\left(|\Pi_n|N_{D}\right) r_n^{3/2}\left[\frac{\lVert \Tilde{\bw}^{n} \rVert_1 \Delta_E  }{\min\{\sqrt{|\Pi_n|},\sqrt{|\mathcal{I}|\}} }  + \Delta^2_E \right] \right) + \frac{r_n\left( 1 + \sqrt{\Delta_E\lVert \Tilde{\bw}^n \rVert_1}\right)}{\sqrt{|\mathcal{I}|}|\Pi_n|^{1/4}}  \right)
%\end{equation}
%\end{lemma}
%\noindent Incorporating the result of the lemma above into \eqref{eq:term2_cauchy_schwarz} gives us
%\begin{align}
%     & \left| \langle \E[\bY_{\mathcal{I}}^{(\pi)}] \nonumber ,\mathcal{P}_{V_{\mathcal{I}}^{(\Pi_n)}}\Delta^n_w \rangle  \right| \\
%     & = O_p \left(\log^{3}\left(|\Pi_n||\mathcal{I}|\right) r_n^{2}\left[\frac{\Delta_E  }{\min\{\sqrt{|\Pi_n|},\sqrt{|\mathcal{I}|\}}}  + \Delta^2_E \right]  + r_n^{3/2}\Delta_E + \frac{r_n\left( 1 + \sqrt{\Delta_E}r^{1/4}_n\right)}{|\Pi_n|^{1/4}}  \right)  \label{eq:Term2_Op_bound}
%\end{align}


==> content/finite_sample_analysis.tex <==
\section{Theoretical Analysis}\label{sec:theoretical_analysis}
%
In this section, we establish finite-sample consistency of \method, starting with a discussion of the additional assumptions required for our results. 

\subsection{Additional Assumptions}\label{subsec:finite_sample_analysis_assumptions}
%
\begin{assumption}[Bounded Potential Outcomes]\label{ass:boundedness_potential_outcome}
We assume that $\E[Y_{n}^{(\pi)}] \in [-1,1]$ for any unit-combination pair $(n,\pi)$.
\end{assumption}
%
\begin{assumption}[Sub-Gaussian Noise]\label{ass:subgaussian_noise}
Conditioned on $\mathcal{A}$, for any unit-combination pair $(n,\pi)$, $\epsilon_n^{\pi}$ are independent zero-mean sub-Gaussian random variables with $\text{Var}[\epsilon_n^{\pi} ~ | ~  \mathcal{A}] \le \sigma^2$ and $\lVert \epsilon_n^{\pi} ~ | ~ \mathcal{A} \rVert_{\psi_2} \leq C\sigma$ for some constant $C > 0$. 
\end{assumption}
%
\begin{assumption} [Incoherence of Donor Fourier characteristics]
\label{ass:incoherence}
For every unit $u \in \mathcal{I}$, assume $\bchi(\Pi_u)$ satisfies incoherence:
$
\left\lVert \frac{\bchi(\Pi_u)^T\bchi(\Pi_u)}{|\Pi_u|} - \mathbf{I}_{2^p}\right\rVert_{\infty} \leq \frac{C'}{s}, 
$ for a universal constant $C' >0$. 
\end{assumption}
%
To define our next set of assumptions, we introduce necessary notation. For any subset of combinations $\Pi_S \subset \Pi$, let $\E[\bY_{\mathcal{I}}^{(\Pi_S)}] = [\E[\bY_u^{(\Pi_S)}]: u \in \mathcal{I}] \in \mathbb{R}^{|\Pi_S| \times |\mathcal{I}|}$.
%
\begin{assumption} [Donor Unit Balanced Spectrum]\label{ass:balanced_spectrum} For a given unit $n \in [N] \setminus \mathcal{I}$, let $r_n$ and $s_{1} \ldots s_{r_n}$ denote the rank and non-zero singular values of $ \E[\bY_{\mathcal{I}}^{(\Pi_n)} \ | \ \mathcal{A}]$, respectively. 
%
We assume that the singular values are well-balanced, i.e., for universal constants $c,c' > 0$, we have that $s_{r_n}/s_{1} \geq c$, and $\lVert \E[\bY^{(\Pi_n)}_{\mathcal{I}} ~ | ~ \mathcal{A} ]\rVert^2_F \geq c'|\Pi_n||\mathcal{I}|$.
\end{assumption}

\begin{assumption} [Subspace Inclusion]\label{ass:rowspace_inclusion} 
For a given unit $n \in [N] \setminus \mathcal{I}$ and intervention $\pi \in \Pi \setminus \Pi_n$,
assume that $\E[\bY^{(\pi)}_{\mathcal{I}}]$ lies within the row-span of $\E[\bY_{\mathcal{I}}^{(\Pi_n)}]$
\end{assumption}
%
\vspace{-2mm}
Assumption \ref{ass:incoherence} is necessary for finite-sample consistency when estimating $\balpha_n$ via the Lasso estimator \eqref{eq:Lasso_estimator}, and is commonly made when studying the Lasso \citep{rigollet2015high}. 
%
Incoherence can also seen as a inclusion criteria for a unit $n$ to be included in the donor set $\mathcal{I}$.  
%
Lemma 2 in \cite{negahban2012learning} shows that the Assumption \ref{ass:incoherence} is satisfied with high probability if $\Pi_u$ is chosen uniformly at random and grows as $\omega(s^2p)$. 
%
If Assumption \ref{ass:incoherence} does not hold, then the Lasso may not estimate $\balpha_u$ accurately, and alternative horizontal regression algorithms may be required instead. 
%
Assumption \ref{ass:balanced_spectrum} requires that the non-zero singular values of $\E[\bY_{\mathcal{I}}^{(\Pi_n)} ~ | ~ \mathcal{A}]$ are well-balanced. 
%
This assumption is standard when studying PCR \cite{agarwal2019robustness,agarwal2020synthetic}, and within the econometrics literature \cite{bai2021matrix,fan2018eigenvector}. 
%
It can also be empirically validated by plotting the spectrum of $\hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n)}]$; if the singular spectrum of $\hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n)}]$ displays a natural elbow point, then Assumption \ref{ass:balanced_spectrum} is likely. 
%
Assumption \ref{ass:rowspace_inclusion} is also commonly made when analyzing PCR \cite{agarwal2020principal,agarwal2020synthetic,agarwal2021causal}.
%
It can be thought of as a ``causal transportability'' condition from the model learnt using $\Pi_n$ to the interventions $\pi \in \Pi \setminus \Pi_n$. 
%
That is, subspace inclusion allows us to generalize well, and accurately estimate $\E[Y_n^{(\pi)} ~ | ~ \mathcal{A} ]$ using $\langle \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n)}], \hat{\bw}^n \rangle$. 
%
In Section \ref{sec:experimental_design}, we propose a simple experimental design mechanism that ensures that Assumptions \ref{ass:incoherence}, \ref{ass:balanced_spectrum}, \ref{ass:rowspace_inclusion} (and Assumption  \ref{ass:donor_set_identification}), i.e., the key conditions for \method~to work, hold with high probability. 
%As we show in Section \ref{sec:experimental_design}, subspace inclusion holds with high probability if $|\Pi_n|$ is chosen uniformly and independently at random from $\Pi$ and has size $\omega(r\log(|\mathcal{I}|))$.
\vspace{-2mm}

\subsection{Finite Sample Consistency}\label{subsec:finite_sample_consistency}
\vspace{-2mm}
%
The following result establishes finite-sample consistency of \method. 
%
Without loss of generality, we will focus on estimating the pair of quantities $(\E[Y_u^{(\pi)}],\E[Y_n^{(\pi)}])$ for a given donor unit $u \in \mathcal{I}$, and non-donor unit $n \in [N] \setminus \mathcal{I}$ under treatment assignment $\pi \in \Pi$.
%
To simplify notation, we will use $O_p$ notation:
%
for any sequence of random vectors $X_n$, $X_n$ = $O_p(\gamma_n)$ if, for any $\epsilon > 0$, there exists constants $c_\epsilon$ and $n_\epsilon$ such that $\mathbb{P}(\lVert X_n \rVert_2 \geq c_\epsilon\gamma_n) \leq \epsilon$ for every $n \geq n_\epsilon$. 
%
Similarly, we define $\tilde{O_p}(\gamma_n)$ which suppresses  logarithmic terms. 
%
We will further absorb dependencies on $\sigma$ into $\tilde{O}_p\left(\cdot\right)$. 
%

\textcolor{blue}{\noindent Moved assumptions to part(a), (b) respectively.}


\begin{theorem} [Finite Sample Consistency of \method]
\label{thm:potential_outcome_convergence_rate}
Conditioned on $\mathcal{A}$, let Assumptions \ref{ass:observation_model}, \ref{ass:selection_on_fourier}, \ref{ass:donor_set_identification}, \ref{ass:boundedness_potential_outcome}, \ref{ass:subgaussian_noise}, and \ref{ass:incoherence} hold. Then, the following statements hold. 
\begin{itemize}
    \item [(a)] For any donor unit-combination pair $(u,\pi)$, let the Lasso regularization parameter satisfy $\lambda_u = \Omega(\sqrt{\frac{p}{|\Pi_u|}})$, then we have that
        $$
            |\hat{\E}[Y_u^{(\pi)}] - \E[Y_{u}^{(\pi)}]| = \Tilde{O}_p\left(\sqrt{\frac{s^2p}{|\Pi_u|}} \right).
        $$
    \item [(b)] Additionally, let Assumptions \ref{ass:balanced_spectrum}, and \ref{ass:rowspace_inclusion} hold. Then, for any non-donor unit-combination pair $(n,\pi)$ where $n \in [N] \setminus \mathcal{I}$, if $\kappa = \text{rank}(\E[\bY_{\mathcal{I}}^{(\Pi_n)}]) \coloneqq r_{n}$, and $ \min_{u \in \mathcal{I}} |\Pi_u| \coloneqq M = \omega(r_n^2s^2p)$, we have that,
        $$
            \left |\hat{\E}[Y_n^{(\pi)}] - \E[Y_{n}^{(\pi)}]\right| = \Tilde{O_p}\left(  \frac{r^2_n\sqrt{s^2p}}{\sqrt{M \times \min\{|\Pi_n|,|\mathcal{I}|\}}} + \frac{r^2_ns^2p\sqrt{|\mathcal{I}|}}{M} + \frac{r_n}{|\Pi_n|^{1/4}}\right).
        $$
\end{itemize}

\end{theorem}
\vspace{-2.5mm}
%
Establishing Theorem \ref{thm:potential_outcome_convergence_rate} requires a novel analysis of error-in-variables (EIV) linear regression.
%
Specifically, the general EIV linear model is as follows: $Y = \bX \beta + \epsilon$, $\mathbf{Z} = \bX + \mathbf{H}$, where $Y$ and $\mathbf{Z}$ are observed.
%
In our case, $Y = \bY_{\Pi_n}$, $\bX = \E[\bY_{\mathcal{I}}^{(\Pi_n)}]$, $\beta = \bw^n$ , $\bZ = \hat{\E}[\bY_{\mathcal{I}}^{(\Pi_n)}]$, and $\mathbf{H}$ is the error arising in estimating $\E[\bY_{\mathcal{I}}^{(\Pi_n)}]$ via the Lasso.
%
Typically one assumes that $\mathbf{H}$ is is a matrix of independent sub-gaussian noise. 
%
Our analysis requires a novel worst-case analysis of $\mathbf{H}$ (due to the 2-step regression of Lasso and then PCR), in which each entry of is  $\mathbf{H}$ simply bounded.

%Previous works assume that $\bH$ is is a matrix of independent sub-gaussian noise. Our analysis requires a worst-case analysis of H (due to the 2-step regression of Lasso and then PCR), which each entry of is H simply bounded. } 
%$\bZ = \bX + \bH$, where $Y$ and $\bZ$ are observed. }


%in our setting, the covariate matrix used in PCR (i.e., $\hat{\E}[Y_{\mathcal{I}}^{(\Pi_n)}]$) is corrupted by bounded noise that arises from estimating potential outcomes via the Lasso for the donor set. This differs from previous work in which the covariate matrix is corrupted by independent sub-gaussian noise. }

Next, we describe the conditions placed on $\Pi_n$, $M$, $\mathcal{I}$ to achieve consistent estimation of $(\E[Y_u^{(\pi)}], \ \E[Y_n^{(\pi)}])$. 
%
To simplify the discussion, we assume that $\min\{|\Pi_n|,|\mathcal{I}|\} = \mathcal{|I|}$. 
%
This condition can be enforced in practice by simply picking a subset of donor units such that $|\mathcal{I}| \leq |\Pi_n|$ when performing PCR (i.e., step 2 of \method).
%
Given this assumption, it can be verified that $|\Pi_n|$ and $M$ need to scale as $\omega(r_n^4)$ and $\omega(r^4_ns^2p)$ respectively to achieve $\max\left(|\hat{\E}[Y_u^{(\pi)}] - \E[Y_{u}^{(\pi)}]|, \ |\hat{\E}[Y_n^{(\pi)}] - \E[Y_{n}^{(\pi)}]|\right) =\tilde{o}_p(1)$.
%
Next, we present a corollary that discusses how quickly the parameters $r_n$, $s$, and $p$ can grow with the number of observations $|\Pi_n|$ and $M$.

{\color{blue}{\noindent Checked conditions for $s,r_n$. Made it more general. }}

{\color{red}
\begin{corollary}\label{cor:potential_outcome_convergence_rate_simplified}
%
With the set-up of Theorem \ref{thm:potential_outcome_convergence_rate}, if the following conditions hold: $r_n = o(|\Pi_n|^{1/4})$, and $s = o\left(\sqrt{\frac{M}{p}} \cdot \min \left(\frac{1}{|\Pi_n|^{1/4}|\mathcal{I}|^{1/4}}, \sqrt{\frac{\min\{|\Pi_n|,|\mathcal{I}|\}}{|\Pi_n|}} \right)\right)$, then 
$
\max\left(|\hat{\E}[Y_u^{(\pi)}] - \E[Y_{u}^{(\pi)}]|, \\ \ |\hat{\E}[Y_n^{(\pi)}] - \E[Y_{n}^{(\pi)}]|\right) =\tilde{o}_p(1) 
$ as $M,|\Pi_n|,|\mathcal{I}| \to \infty$. 
%
\end{corollary}
}
\vspace{-1.5mm}
%
\noindent Corollary \ref{cor:potential_outcome_convergence_rate_simplified} quantifies how $s, r_n$ can scale with the number of observations to achieve consistency. 
%
That is, Corollary \ref{cor:potential_outcome_convergence_rate_simplified} reflects the maximum ``complexity'' allowed for a given sample size. 

\subsection{Finite-Sample Consistency of CART}
\label{subsec:CART_finite_sample}

{\color{blue}{Rewrote most of section, so did not highlight in red.}}

\noindent As discussed in Section \ref{sec:estimator_descripton}, \method~allows for any ML algorithm to be used for horizontal regression. 
%
In this section, we present theoretical results when the horizontal regression is done via CART. 
%
We show that when the potential outcome function is a $k$-Junta (see equation \eqref{eq:k_junta} for the definition), CART is able to achieve stronger sample complexity guarantees than the Lasso. 
%
We refer the reader to Appendix \ref{sec:CART_horizontal_regression} for a description of the CART algorithm.
%
Our CART-based horizontal regression procedure consists of the following two steps. 


\noindent \textbf{Step 1: Feature Identification.} For each donor unit $u \in \mathcal{I}$, divide the observed interventions $\Pi_u$ equally into two sets $\Pi^{a}_u$ and $\Pi^{b}_u$. Fit a CART model $\mathcal{\hat{T}}$ on the dataset $\mathcal{D}^a_u = [\{\bv(\pi),Y_{u\pi}\}: \pi \in \Pi^a_u]$. Let $\hat{K}_u = \{\bv(\pi)_j : \bv(\pi)_j$ $\in \mathcal{\hat{T}}\}$ denote every feature that the CART splits on. 

\noindent \textbf{Step 2: Estimation.} For every subset $S \subset \hat{K}_u$, compute $\hat{\alpha}_{u,S} = \frac{1}{|\Pi^b_u|}\sum_{\pi \in \Pi^b_u }Y_{u\pi}\chi^{\pi}_{S}$. We then estimate our target causal parameter as follows: $\hat{\E}[Y_u^{(\pi)}] = \sum_{S \in \hat{K}_u}\hat{\alpha}_{u,S}\chi^{\pi}_{S}$.

\noindent CART is able to take advantage of the $k$-Junta structure of the potential outcomes by first performing feature selection (i.e., learning the relevant feature set $\hat{K}_u$), before estimating the Fourier coefficient for each relevant subset.
%
In contrast, Lasso estimates the Fourier coefficient of all $2^p$ subsets simultaneously. 
%

Next, we present our theoretical results that establishes CART exploits this $k$-Junta structure to provide better sample complexity guarantees than the Lasso.
%
Specifically, we present an informal theorem for the horizontal regression finite sample error when the horizontal regression is done via CART.  
%
The formal result (Theorem \ref{thm:CART_convergence_rate}) can be found in Appendix \ref{subsec:CART_finite_sample}.

\begin{theorem} [Informal]
\label{thm:informal_CART_potential_outcome_convergence_rate}
For a given donor unit $u$, suppose $\E[Y_u^{(\pi)}]$ is a $k$-Junta, then, if the horizontal regression is done via CART, we have
        $
            |\hat{\E}[Y_u^{(\pi)}] - \E[Y_{u}^{(\pi)}]| = \Tilde{O}_p\left(\sqrt{\frac{s^2}{|\Pi_u|}} \right).
       $
\end{theorem}
%
Compared to the Lasso horizontal regression error (see Theorem \ref{thm:potential_outcome_convergence_rate} (a)), CART removes an additional factor of $p$ by exploiting the $k$-Junta structure. 
%
As a result, it can be verified that CART also removes a factor of $p$ for the vertical regression error (see Theorem \ref{thm:potential_outcome_convergence_rate} (b)). 
%
Next, we describe the conditions required for $\Pi_n$, $M$, $\mathcal{I}$ to consistently estimate $(\E[Y_u^{(\pi)}], \ \E[Y_n^{(\pi)}])$ for a given donor unit $u$, non-donor unit $n$, and combination $\pi$ with \method~when the horizontal regression is done via CART.
%
Like the discussion after Theorem \ref{thm:potential_outcome_convergence_rate}, we assume  $\min\{|\Pi_n|,|\mathcal{I}|\} = \mathcal{|I|}$ to simplify the discussion. 
%
Given this assumption, it can be verified that $|\Pi_n|$ and $M$ need to scale as $\omega(r_n^4)$ and $\omega(r^4_ns^2)$ respectively to achieve $\max\left(|\hat{\E}[Y_u^{(\pi)}] - \E[Y_{u}^{(\pi)}]|, \ |\hat{\E}[Y_n^{(\pi)}] - \E[Y_{n}^{(\pi)}]|\right) =\tilde{o}_p(1)$.
%
That is, CART reduces the number of required observations for donor units by a factor of $p$.



%\begin{corollary}
%\label{cor:potential_outcome_convergence_rate_CART}
%
%Let the set-up of Theorems \ref{thm:potential_outcome_convergence_rate}, \ref{thm:CART_convergence_rate}, and condition (a) of Corollary \ref{cor:potential_outcome_convergence_rate_simplified} hold. 
%
%Then, if $s =  o\left(\sqrt{M/(\max\{|\Pi_n|,|\mathcal{I}|\}})\right)$, 
%$\max\left(|\hat{\E}[Y_u^{(\pi)}] - \E[Y_{u}^{(\pi)}]|, \ |\hat{\E}[Y_n^{(\pi)}] - \E[Y_{n}^{(\pi)}]|\right) =\tilde{o}_p(1)$
%
%\end{corollary} 
%\vspace{-2mm}
%
%\noindent Corollary \ref{cor:potential_outcome_convergence_rate_CART} 
%shows CART can achieve consistency while allowing the sparsity $s$ to scale more quickly (i.e., by a factor of $p$) than the Lasso. 
%
%That is, CART exploits the additional regularity conditions placed on the potential outcomes to achieve consistency with $M = \omega(r_n^4s^2)$ samples. 
%
%As discussed above, the superior sample complexity of CART arises from the fact that it identifies the relevant feature subset before estimating the Fourier coefficient.
%

%shows CART exploits the additional regularity conditions placed on the potential outcomes to allow the sparsity $s$ to scale more quickly (i.e., by a factor of $p$) while maintaining consistency. 



\subsection{Sample Complexity}
\label{subsec:sample_complexity_synth_combo}
\vspace{-2.5mm}
We discuss the sample complexity of \method~to estimate all $N \times 2^p$ causal parameters, and compare it to that of other methods.
%
To ease our discussion, we will ignore dependence on logarithmic factors.
%
Again, we assume that the horizontal regression is done via the Lasso. 

%
Even if potential outcomes $Y_n^{(\pi)}$ were observed for all unit-combination pairs, consistently estimating $\E[\bY_N^{(\Pi)}]$ is not trivial. 
%
This is because, we only get to observe a single and noisy version $Y_{n\pi} = \langle \balpha_n, \bchi^{\pi} \rangle + \epsilon_n^{\pi}$. 
%
Hypothetically, if we observe $K$ independent samples of $Y_{n\pi}$ for a given $(n,\pi)$, denoted by $Y^{1}_{n\pi}, \ldots, Y^{K}_{n\pi}$, the maximum likelihood estimator would be the empirical average $\frac{1}{K}\sum^K_{i=1}Y^{i}_{n\pi}$. 
%
The empirical average would concentrate around $\E[Y_n^{(\pi)}]$ at a rate $O(1/\sqrt{K})$ and hence would require $K = \Omega(\delta^{-2})$ samples to estimate $\E[Y_n^{(\pi)}]$ within error $O(\delta)$. 
%
Therefore, this naive (unimplementable) solution would require $N \times 2^p \times \delta^{-2}$ observations to estimate $\E[\bY_N^{(\Pi)}]$. 
%

On the other hand, \method~produces consistent estimates of the potential outcome despite being given {\em at most only a single noisy sample} of each potential outcome. 
%
As the discussion after Theorem \ref{thm:potential_outcome_convergence_rate} shows, if $|\mathcal{I}| \leq |\Pi_n|$, \method~requires $|\mathcal{I}| \times r^4s^2p/\delta^2$ observations for the donor set, and $(N - |\mathcal{I}|) \times r^4/\delta^4$ observations for the non-donor units to achieve an estimation error of $O(\delta)$ for all $N \times 2^p$ causal parameters. 
%
Hence, we have that the number of observations required to achieve an estimation error of $O(\delta)$ for all pairs $(n,\pi)$  scales as $O\left(\text{poly}(r/\delta) \times \left(N + s^2p \right) \right)$.
%Hence, at most $N \times r^4/\delta^4$ + $|\mathcal{I}| \times r^4s^2p/\delta^2$ observations are required to estimate $\E[Y_n^{(\pi)}]$ with error $O(\delta)$ for all pairs $(n,\pi)$. 
%
%Of course, this is assuming that the key assumptions (see Section \ref{subsec:finite_sample_analysis_assumptions}) are satisfied. 
%
%Hence, we have that the number of observations required to achieve an estimation error of $O(\delta)$ scales as $O\left(\text{poly}(r)/\delta^4 \times \left(N + s^2p \right) \right)$. 
%

\vspace{2mm}
\noindent \textbf{Sample Complexity Comparison to Other Methods.}  

\noindent \emph{Horizontal regression:} An alternative algorithm would be to learn an individual model for each unit $n \in [N]$. 
%
That is, run a separate horizontal regression via the Lasso for every unit.
%
This alternative algorithm has sample complexity that scales at least as $O(N \times s^2p/\delta^2)$  rather than $O\left(\text{poly}(r)/\delta^4  \times \left(N + s^2p \right) \right)$ required by \method.  
%
It suffers because it does not utilize any structure across units (i.e., the low-rank property of $\mathcal{A}$), whereas \method~captures the similarity between units via PCR. 
%

\vspace{1mm}
\noindent \emph{Matrix completion:} \method~can be thought of as a matrix completion method; estimating $\E[Y_n^{(\pi)}]$ is equivalent to imputing $(n,\pi)$-th entry of the observation matrix $\bY \in \{\mathbb{R} \cup \star\}^{N \times 2^p}$, where recall $\star$ denotes an unobserved unit-combination outcome. 
%
Under the low-rank property (Assumption \ref{ass:observation_model}(b)) and various models of missingness (i.e., observation patterns), recent works on matrix completion \cite{candes2010matrix,ma2019missing,agarwal2021causalmatrix} (see Section \ref{sec:related_work} for an overview) have established that estimating $\E[Y_n^{(\pi)}]$ to an accuracy $O(\delta)$ requires at least $O\left(\text{poly}(r/\delta) \times \left(N + 2^p \right)\right)$ samples.
%
This is because matrix completion techniques do not leverage the sparsity of $\balpha_n$.
%leverage additional structural information such as the Fourier expansion of Boolean functions and the resulting sparsity in $\balpha_n$.
%
Moreover,
matrix completion results typically report error in the Frobenius norm, whereas we give entry-wise guarantees. 
%
This leads to an extra factor of $s$ in our analysis as it requires proving convergence for $\lVert \hat{\balpha_n} - \balpha_n \rVert_{1}$ rather than $\lVert \hat{\balpha_n} - \balpha_n \rVert_{2}$. 
%
Hence, \method~combines the best of both approaches by leveraging both the structure of the potential outcomes \emph{and} the similarity across units. 

\vspace{2mm}
\noindent \textbf{Natural Lower Bound on Sample Complexity.} We provide an informal discussion on the lower bound sample-complexity to estimate all $N \times 2^p$ potential outcomes. 
%
As established in Lemma \ref{lem:number_nonzeros}, $\mathcal{A}$ has at most $rs$ non-zero columns. 
%
Counting the parameters in the singular value decomposition of $\mathcal{A}$, only $r\times (N + rs)$ free parameters are required to be estimated. 
%
Hence, a natural lower bound on the sample complexity scales as $O(Nr + r^2s)$.  
%
Hence, \method~is only sub-optimal by a factor (ignoring logarithmic factors) of $sp$ and $\text{poly}(r)$.  
%
As discussed earlier, an additional factor of $s$ can be removed if we focus on deriving Frobenius norm error bounds.
%
Further, the use of non-linear methods such as CART can remove the factor of $p$ (Theorem \ref{thm:informal_CART_potential_outcome_convergence_rate}) under stronger assumptions on the potential outcomes such as when $\E[Y_n^{(\pi)])}]$ is a $k$-Junta that satisfies regularity conditions. 
%
It remains interesting future work to derive estimation procedures that are able to achieve this lower bound.



%Next, we present a corollary analogous to Corollary \ref{cor:potential_outcome_convergence_rate_simplified} that discusses how quickly 
%that assumes the horizontal regression is done via CART instead. 



%present the additional assumptions required on the potential outcomes for finite-sample consistency of \method~when using CART instead of Lasso. 
%
%We only present an informal discussion of these assumptions, and leave the precise formulation to Appendix \textcolor{red}{H}.  

% how quickly the parameters $r_n,s,p$ are allowed to grow with the number of observations $|\Pi_n|$, and $M$ for \method~with CART to achieve consistency. 

% o\left(\sqrt{M/(p\max\{|\Pi_n|,|\mathcal{I}|\}})\right) $




%for estimating our target causal parameter via \method.  
%
%{\color{red} Specifically, we establish a corollary analogous to Corollary \ref{cor:potential_outcome_convergence_rate_simplified} that quantifies the maximum complexity (as measured by $r_n,s,p$) allowed by CART for a given sample size. 
%
%Before presenting the corollary, we provide an informal discussion of the assumptions imposed on the potential outcomes $\E[Y_n^{(\pi)}]$ required for CART to achieve finite-sample consistency. 
%
%We assume: (i) $\E[Y_n^{(\pi)}]$ is a $k$-Junta as discussed above, (ii) $\E[Y_n^{(\pi)}]$ satisfies a ``sub-modularity'' condition which is necessary for greedy-tree algorithms such as CART to achieve consistency (see Definition \ref{def:strong_partition_sparsity} for an exact characterization of this sub-modularity condition), and (iii) the combinations of donor units are observed uniformly at random. 
%
%Given this discussion on the required assumptions, we present our theoretical result as follows.}
